The Future of US Particle Physics -- The Snowmass 2021 Energy Frontier Report

This report, as part of the 2021 Snowmass Process, summarizes the current status of collider physics at the Energy Frontier, the broad and exciting future prospects identified for the Energy Frontier, the challenges and needs of future experiments, and indicates high priority research areas.

==> Energy/Energy.bib.220610 <==


@article{McCullough:2013rea,
    author = "McCullough, Matthew",
    title = "{An Indirect Model-Dependent Probe of the Higgs Self-Coupling}",
    eprint = "1312.3322",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4521",
    doi = "10.1103/PhysRevD.90.015001",
    journal = "Phys. Rev. D",
    volume = "90",
    number = "1",
    pages = "015001",
    year = "2014",
    note = "[Erratum: Phys.Rev.D 92, 039903 (2015)]"
}

@article{Baldenegro:2018hng,
    author = "Baldenegro, Cristian and Fichet, Sylvain and von Gersdorff, Gero and Royon, Christophe",
    title = "{Searching for axion-like particles with proton tagging at the LHC}",
    eprint = "1803.10835",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP06(2018)131",
    journal = "JHEP",
    volume = "06",
    pages = "131",
    year = "2018"
}

@article{Baldenegro:2022kaa,
    author = "Baldenegro, Cristian and Bellora, Andrea and Fichet, Sylvain and von Gersdorff, Gero and Pitt, Michael and Royon, Christophe",
    title = "{Searching for anomalous top quark interactions with proton tagging and timing detectors at the LHC}",
    eprint = "2205.01173",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "5",
    year = "2022"
}

@article{Baldenegro:2017aen,
    author = "Baldenegro, Cristian and Fichet, Sylvain and von Gersdorff, Gero and Royon, Christophe",
    title = "{Probing the anomalous \ensuremath{\gamma}\ensuremath{\gamma}\ensuremath{\gamma}Z coupling at the LHC with proton tagging}",
    eprint = "1703.10600",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP06(2017)142",
    journal = "JHEP",
    volume = "06",
    pages = "142",
    year = "2017"
}

@article{Fichet:2014uka,
    author = "Fichet, Sylvain and von Gersdorff, Gero and Lenzi, Bruno and Royon, Christophe and Saimpert, Matthias",
    title = "{Light-by-light scattering with intact protons at the LHC: from Standard Model to New Physics}",
    eprint = "1411.6629",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP02(2015)165",
    journal = "JHEP",
    volume = "02",
    pages = "165",
    year = "2015"
}

@article{Fichet:2013gsa,
    author = "Fichet, S. and von Gersdorff, G. and Kepka, O. and Lenzi, B. and Royon, C. and Saimpert, M.",
    title = "{Probing new physics in diphoton production with proton tagging at the Large Hadron Collider}",
    eprint = "1312.5153",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.89.114004",
    journal = "Phys. Rev. D",
    volume = "89",
    pages = "114004",
    year = "2014"
}

@article{Fichet:2016pvq,
    author = "Fichet, Sylvain and von Gersdorff, Gero and Royon, Christophe",
    title = "{Measuring the Diphoton Coupling of a 750 GeV Resonance}",
    eprint = "1601.01712",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.116.231801",
    journal = "Phys. Rev. Lett.",
    volume = "116",
    number = "23",
    pages = "231801",
    year = "2016"
}

@article{Fichet:2015vvy,
    author = "Fichet, Sylvain and von Gersdorff, Gero and Royon, Christophe",
    title = "{Scattering light by light at 750 GeV at the LHC}",
    eprint = "1512.05751",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.93.075031",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "7",
    pages = "075031",
    year = "2016"
}

@article{Chapon:2009hh,
    author = "Chapon, E. and Royon, C. and Kepka, O.",
    title = "{Anomalous quartic W W gamma gamma, Z Z gamma gamma, and trilinear WW gamma couplings in two-photon processes at high luminosity at the LHC}",
    eprint = "0912.5161",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.81.074003",
    journal = "Phys. Rev. D",
    volume = "81",
    pages = "074003",
    year = "2010"
}

@article{Kepka:2008yx,
    author = "Kepka, O. and Royon, C.",
    title = "{Anomalous $W W \gamma$ coupling in photon-induced processes using forward detectors at the LHC}",
    eprint = "0808.0322",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.78.073005",
    journal = "Phys. Rev. D",
    volume = "78",
    pages = "073005",
    year = "2008"
}

@article{Baldenegro:2019whq,
    author = "Baldenegro, C. and Hassani, S. and Royon, C. and Schoeffel, L.",
    title = "{Extending the constraint for axion-like particles as resonances at the LHC and laser beam experiments}",
    eprint = "1903.04151",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physletb.2019.06.029",
    journal = "Phys. Lett. B",
    volume = "795",
    pages = "339--345",
    year = "2019"
}

@article{LGAD,
    author = "Barletta, P. and Cerullo, M. and Haber, C. and Holland, S. E. and Muth, J. and Sekely, B.",
    title = "{Fast Timing With Silicon Carbide Low Gain Avalanche Detectors}",
    eprint = "2203.08554",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "3",
    year = "2022"
}

@techreport{HIG-21-008-pas,
      title         = "{Direct search for the standard model Higgs boson decaying
                       to a charm quark-antiquark pair}",
      collaboration = "CMS",
      reportNumber  = "CMS-PAS-HIG-21-008",
      year          = "2022",
}

@article{CMS:2020xrn,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{A measurement of the Higgs boson mass in the diphoton decay channel}",
    eprint = "2002.06398",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-HIG-19-004, CERN-EP-2020-004",
    doi = "10.1016/j.physletb.2020.135425",
    journal = "Phys. Lett. B",
    volume = "805",
    pages = "135425",
    year = "2020"
}


@article{ATLAS:2020coj,
    author = "{ATLAS Collaboration}",
    title = "{Measurement of the Higgs boson mass in the $H \rightarrow ZZ^* \rightarrow 4\ell$ decay channel with $\sqrt{s}=13$ TeV $pp$ collisions using the ATLAS detector at the LHC}",
    reportNumber = "ATLAS-CONF-2020-005, ATLAS-CONF-2020-005",
    month = "4",
    year = "2020"
}


@article{ATLAS:2020qdt,
    collaboration = "ATLAS",
    title = "{A combination of measurements of Higgs boson production and decay using up to $139$ fb$^{-1}$ of proton--proton collision data at $\sqrt{s}=$ 13 TeV collected with the ATLAS experiment}",
    reportNumber = "ATLAS-CONF-2020-027",
    month = "8",
    year = "2020"
}


@article{CMS:2020gsy,
    collaboration = "CMS",
    title = "{Combined Higgs boson production and decay measurements with up to 137 fb$^{-1}$ of proton-proton collision data at $\sqrt s$ = 13 TeV}",
    reportNumber = "CMS-PAS-HIG-19-005",
    year = "2020"
}


@article{CMS:2022qva,
    author = "Tumasyan, Armen and others",
    collaboration = "CMS",
    title = "{Search for invisible decays of the Higgs boson produced via vector boson fusion in proton-proton collisions at $\sqrt{s} =$ 13 TeV}",
    eprint = "2201.11585",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-HIG-20-003, CERN-EP-2021-273",
    doi = "10.1103/PhysRevD.105.092007",
    journal = "Phys. Rev. D",
    volume = "105",
    pages = "092007",
    year = "2022"
}


@article{CMS:2020xwi,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Evidence for Higgs boson decay to a pair of muons}",
    eprint = "2009.04363",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-HIG-19-006, CERN-EP-2020-164",
    doi = "10.1007/JHEP01(2021)148",
    journal = "JHEP",
    volume = "01",
    pages = "148",
    year = "2021"
}


@article{CMS:2020tkr,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Search for nonresonant Higgs boson pair production in final states with two bottom quarks and two photons in proton-proton collisions at $ \sqrt{s} $ = 13 TeV}",
    eprint = "2011.12373",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-HIG-19-018, CERN-EP-2020-222",
    doi = "10.1007/JHEP03(2021)257",
    journal = "JHEP",
    volume = "03",
    pages = "257",
    year = "2021"
}


@article{CMS:2022cpr,
    author = "Tumasyan, Armen and others",
    collaboration = "CMS",
    title = "{Search for Higgs boson pair production in the four b quark final state in proton-proton collisions at $\sqrt{s}$ = 13 TeV}",
    eprint = "2202.09617",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-HIG-20-005, CERN-EP-2022-004",
    month = "2",
    year = "2022"
}


@article{ATLAS-CONF-2021-052,
    collaboration = "ATLAS",
    title = "{Combination of searches for non-resonant and resonant Higgs boson pair production in the $b\bar{b}\gamma\gamma$, $b\bar{b}\tau^{+}\tau^{-}$ and $b\bar{b}b\bar{b}$ decay channels using $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector}",
    reportNumber = "ATLAS-CONF-2021-052",
    year = "2021"
}


@inproceedings{Dasu:2022nux,
    author = "Dasu, Sridhara and others",
    title = "{Strategy for Understanding the Higgs Physics: The Cool Copper Collider}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07646",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "SLAC-PUB-17661, FERMILAB-CONF-22-311-AD-PPD-SCD-SQMS-TD",
    month = "3",
    year = "2022"
}


@article{Fujii:2018mli,
    author = "Fujii, Keisuke and others",
    title = "{The role of positron polarization for the inital $250$ GeV stage of the International Linear Collider}",
    eprint = "1801.02840",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-237, KEK-PREPRINT-2017-57, SLAC-PUB-17197",
    month = "1",
    year = "2018"
}


@article{Barklow:2017suo,
    author = "Barklow, Tim and Fujii, Keisuke and Jung, Sunghoon and Karl, Robert and List, Jenny and Ogawa, Tomohisa and Peskin, Michael E. and Tian, Junping",
    title = "{Improved Formalism for Precision Higgs Coupling Fits}",
    eprint = "1708.08912",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-120, KEK-PREPRINT-2017-22, SLAC-PUB-17129",
    doi = "10.1103/PhysRevD.97.053003",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "5",
    pages = "053003",
    year = "2018"
}


@inproceedings{MuonCollider:2022xlm,
    author = "de Blas, Jorge and others",
    collaboration = "Muon Collider",
    title = "{The physics case of a 3 TeV muon collider stage}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07261",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-22-317-AD-ND-PPD-SCD-TD",
    month = "3",
    year = "2022"
}


@article{ATL-PHYS-PUB-2022-018,
    collaboration = "ATLAS",
    title = "{Snowmass White Paper Contribution: Physics with the Phase-2 ATLAS and CMS Detectors}",
    reportNumber = "ATL-PHYS-PUB-2022-018",
    year = "2022"
}


@article{ATL-PHYS-PUB-2022-005,
    collaboration = "ATLAS",
    title = "{Projected sensitivity of Higgs boson pair production combining the $b\bar{b}\gamma\gamma$ and $b\bar{b}\tau^{+}\tau^{-}$ final states with the ATLAS detector at the HL-LHC}",
    reportNumber = "ATL-PHYS-PUB-2022-005",
    year = "2022"
}


@article{ILCInternationalDevelopmentTeam:2022izu,
    collaboration = "ILC International Development Team",
    title = "{The International Linear Collider: Report to Snowmass 2021}",
    eprint = "2203.07622",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "DESY-22-045, IFT-UAM/CSIC-22-028, KEK Preprint 2021-61, SLAC-PUB-17662, FERMILAB-FN-1171-PPD-QIS-SCD-TD, PNNL-SA-160884",
    month = "3",
    year = "2022"
}


@article{Robson:2018zje,
    author = "Robson, Aidan and Roloff, Philipp",
    title = "{Updated CLIC luminosity staging baseline and Higgs coupling prospects}",
    eprint = "1812.01644",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CLICdp-Note-2018-002",
    month = "12",
    year = "2018"
}


@article{Bernardi:2022hny,
    author = "Bernardi, G. and others",
    title = "{The Future Circular Collider: a Summary for the US 2021 Snowmass Process}",
    eprint = "2203.06520",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "3",
    year = "2022"
}


@article{Mangano:2020sao,
    author = "Mangano, Michelangelo L. and Ortona, Giacomo and Selvaggi, Michele",
    title = "{Measuring the Higgs self-coupling via Higgs-pair production at a 100 TeV p-p collider}",
    eprint = "2004.03505",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-052",
    doi = "10.1140/epjc/s10052-020-08595-3",
    journal = "Eur. Phys. J. C",
    volume = "80",
    number = "11",
    pages = "1030",
    year = "2020"
}


@article{deBlas:2019rxi,
    author = "de Blas, J. and others",
    title = "{Higgs Boson Studies at Future Particle Colliders}",
    eprint = "1905.03764",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-19-079",
    doi = "10.1007/JHEP01(2020)139",
    journal = "JHEP",
    volume = "01",
    pages = "139",
    year = "2020"
}


@inproceedings{Abu-Ajamieh:2022dtm,
    author = "Abu-Ajamieh, Fayez and Chang, Spencer and Chen, Miranda and Liu, Da and Luty, Markus A.",
    title = "{Snowmass 2021 White Paper: Higgs Coupling Sensitivities and Model-Independent Bounds on the Scale of New Physics}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.09512",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@inproceedings{Adhikari:2022yaa,
    author = "Adhikari, Shekhar and Lane, Samuel D. and Lewis, Ian M. and Sullivan, Matthew",
    title = "{Complex Scalar Singlet Model Benchmarks for Snowmass}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07455",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@article{deBlas:2017xtg,
    author = "de Blas, J. and Criado, J. C. and Perez-Victoria, M. and Santiago, J.",
    title = "{Effective description of general extensions of the Standard Model: the complete tree-level dictionary}",
    eprint = "1711.10391",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2017-251",
    doi = "10.1007/JHEP03(2018)109",
    journal = "JHEP",
    volume = "03",
    pages = "109",
    year = "2018"
}


@article{Degrassi:2012ry,
    author = "Degrassi, Giuseppe and Di Vita, Stefano and Elias-Miro, Joan and Espinosa, Jose R. and Giudice, Gian F. and Isidori, Gino and Strumia, Alessandro",
    title = "{Higgs mass and vacuum stability in the Standard Model at NNLO}",
    eprint = "1205.6497",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2012-134, RM3-TH-12-9",
    doi = "10.1007/JHEP08(2012)098",
    journal = "JHEP",
    volume = "08",
    pages = "098",
    year = "2012"
}


@article{CDF:2016vzt,
    collaboration = "CDF, D0",
    title = "{Combination of CDF and D0 results on the mass of the top quark using up $9.7\:{\rm fb}^{-1}$ at the Tevatron}",
    eprint = "1608.01881",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-CONF-16-298-E",
    month = "8",
    year = "2016"
}


@article{ATLAS:2018fwq,
    author = "Aaboud, Morad and others",
    collaboration = "ATLAS",
    title = "{Measurement of the top quark mass in the $t\bar{t}\rightarrow $ lepton+jets channel from $\sqrt{s}=8$  TeV ATLAS data and combination with previous results}",
    eprint = "1810.01772",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2018-238",
    doi = "10.1140/epjc/s10052-019-6757-9",
    journal = "Eur. Phys. J. C",
    volume = "79",
    number = "4",
    pages = "290",
    year = "2019"
}


@article{CMS:2015lbj,
    author = "Khachatryan, Vardan and others",
    collaboration = "CMS",
    title = "{Measurement of the top quark mass using proton-proton data at ${\sqrt{(s)}}$ = 7 and 8 TeV}",
    eprint = "1509.04044",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-TOP-14-022, CERN-PH-EP-2015-234",
    doi = "10.1103/PhysRevD.93.072004",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "7",
    pages = "072004",
    year = "2016"
}


@article{ATLAS:2019ezb,
    collaboration = "ATLAS",
    title = "{Measurement of the top quark mass using a leptonic invariant mass in $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector}",
    reportNumber = "ATLAS-CONF-2019-046",
    month = "10",
    year = "2019"
}


@article{CMS:2018tye,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Measurement of the top quark mass in the all-jets final state at $\sqrt{s} =$ 13 TeV and combination with the lepton+jets channel}",
    eprint = "1812.10534",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-TOP-17-008, CERN-EP-2018-310",
    doi = "10.1140/epjc/s10052-019-6788-2",
    journal = "Eur. Phys. J. C",
    volume = "79",
    number = "4",
    pages = "313",
    year = "2019"
}


@article{CMS-PAS-FTR-16-006,
    collaboration = "CMS",
    title = "{ECFA 2016: Prospects for selected standard model measurements with the CMS experiment at the High-Luminosity LHC}",
    reportNumber = "CMS-PAS-FTR-16-006",
    year = "2017"
}


@inproceedings{Czakon:2016teh,
    author = "Czakon, M. and Fiedler, P. and Heymes, D. and Mitov, A.",
    collaboration = "D0",
    title = "{Measurement of the Pole Mass of the Top Quark using Differential $t\bar{t}$ Cross Sections in $p\bar{p}$ Collisions at $\sqrt{s}$ = 1.96 TeV}",
    reportNumber = "FERMILAB-CONF-16-383-PPD, CAVENDISH-HEP-16-15, TTK-16-36, D0-NOTE-6473-CONF",
    month = "9",
    year = "2016"
}


@article{ATLAS:2019guf,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{Measurement of the top-quark mass in $t\bar{t}+1$-jet events collected with the ATLAS detector in $pp$ collisions at $\sqrt{s}=8$ TeV}",
    eprint = "1905.02302",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2019-059",
    doi = "10.1007/JHEP11(2019)150",
    journal = "JHEP",
    volume = "11",
    pages = "150",
    year = "2019"
}


@article{CMS:2019esx,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Measurement of $\mathrm{t\bar t}$ normalised multi-differential cross sections in pp collisions at $\sqrt s=13$ TeV, and simultaneous determination of the strong coupling strength, top quark pole mass, and parton distribution functions}",
    eprint = "1904.05237",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-TOP-18-004, CERN-EP-2019-028",
    doi = "10.1140/epjc/s10052-020-7917-7",
    journal = "Eur. Phys. J. C",
    volume = "80",
    number = "7",
    pages = "658",
    year = "2020"
}


@article{CMS:2018nqq,
    collaboration = "CMS",
    title = "{Projections of sensitivities for tttt production at HL-LHC and HE-LHC}",
    reportNumber = "CMS-PAS-FTR-18-031",
    year = "2018"
}


@article{ATLAS:2022kld,
    collaboration = "ATLAS",
    title = "{Extrapolation of ATLAS sensitivity to the measurement of the Standard Model four top quark cross section at the HL-LHC}",
    reportNumber = "ATL-PHYS-PUB-2022-004",
    year = "2022"
}


@article{Baer:2013cma,
    editor = "Baer, Howard and others",
    title = "{The International Linear Collider Technical Design Report - Volume 2: Physics}",
    eprint = "1306.6352",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ILC-REPORT-2013-040, ANL-HEP-TR-13-20, BNL-100603-2013-IR, IRFU-13-59, CERN-ATS-2013-037, COCKCROFT-13-10, CLNS-13-2085, DESY-13-062, FERMILAB-TM-2554, IHEP-AC-ILC-2013-001, INFN-13-04-LNF, JAI-2013-001, JINR-E9-2013-35, JLAB-R-2013-01, KEK-REPORT-2013-1, KNU-CHEP-ILC-2013-1, LLNL-TR-635539, SLAC-R-1004, ILC-HIGRADE-REPORT-2013-003",
    month = "6",
    year = "2013"
}


@article{Bambade:2019fyw,
    author = "Bambade, Philip and others",
    title = "{The International Linear Collider: A Global Project}",
    eprint = "1903.01629",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "DESY 19-037, DESY-19-037, FERMILAB-FN-1067-PPD, IFIC/19-10, IRFU-19-10,
  JLAB-PHY-19-2854, KEK Preprint 2018-92, JLAB-PHY-19-2854, KEK
  Preprint 2018-92, LAL/RT 19-001, PNNL-SA-142168,
  SLAC-PUB-17412, SLAC-PUB-17412",
    month = "3",
    year = "2019"
}


@article{Linssen:2012hp,
    editor = "Linssen, Lucie and Miyamoto, Akiya and Stanitzki, Marcel and Weerts, Harry",
    title = "{Physics and Detectors at CLIC: CLIC Conceptual Design Report}",
    eprint = "1202.5940",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-2012-003, ANL-HEP-TR-12-01, DESY-12-008, KEK-REPORT-2011-7",
    doi = "10.5170/CERN-2012-003",
    month = "2",
    year = "2012"
}


@article{Charles:2018vfv,
    author = "Charles, T. K. and others",
    editor = "Burrows, P. N. and Catalan Lasheras, N. and Linssen, L. and Petri\v{c}, M. and Robson, A. and Schulte, D. and Sicking, E. and Stapnes, S.",
    collaboration = "CLICdp, CLIC",
    title = "{The Compact Linear Collider (CLIC) - 2018 Summary Report}",
    eprint = "1812.06018",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "CERN-2018-005-M, CERN-2018-005",
    doi = "10.23731/CYRM-2018-002",
    volume = "2/2018",
    month = "12",
    year = "2018"
}


@article{Abada:2019zxq,
    author = "Abada, A. and others",
    collaboration = "FCC",
    title = "{FCC-ee: The Lepton Collider}: {Future Circular Collider Conceptual Design Report Volume 2}",
    reportNumber = "CERN-ACC-2018-0057",
    doi = "10.1140/epjst/e2019-900045-4",
    journal = "Eur. Phys. J. ST",
    volume = "228",
    number = "2",
    pages = "261--623",
    year = "2019"
}


@article{CEPCStudyGroup:2018ghi,
    author = "Dong, Mingyi and others",
    editor = "Guimar\~aes da Costa, Jo\~ao Barreiro and others",
    collaboration = "CEPC Study Group",
    title = "{CEPC Conceptual Design Report: Volume 2 - Physics \& Detector}",
    eprint = "1811.10545",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "IHEP-CEPC-DR-2018-02, IHEP-EP-2018-01, IHEP-TH-2018-01",
    month = "11",
    year = "2018"
}


@inproceedings{Cheng:2022zyy,
    author = "Cheng, Huajie and others",
    collaboration = "CEPC Physics Study Group",
    title = "{The Physics potential of the CEPC. Prepared for the US Snowmass Community Planning Exercise (Snowmass 2021)}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2205.08553",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "5",
    year = "2022"
}


@article{DeBlas:2019qco,
    author = "De Blas, Jorge and Durieux, Gauthier and Grojean, Christophe and Gu, Jiayin and Paul, Ayan",
    title = "{On the future of Higgs, electroweak and diboson measurements at lepton colliders}",
    eprint = "1907.04311",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-19-077, DESY 19-077, HU-EP-19/33, MITP/19-028",
    doi = "10.1007/JHEP12(2019)117",
    journal = "JHEP",
    volume = "12",
    pages = "117",
    year = "2019"
}


@article{LCCPhysicsWorkingGroup:2019fvj,
    author = "Fujii, Keisuke and others",
    collaboration = "LCC Physics Working Group",
    title = "{Tests of the Standard Model at the International Linear Collider}",
    eprint = "1908.11299",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "DESY 19-146, KEK Preprint 2019-22, SLAC-PUB-17467, DESY-19-146",
    month = "8",
    year = "2019"
}


@article{Blondel:2021ema,
    author = "Blondel, Alain and Janot, Patrick",
    title = "{FCC-ee overview: new opportunities create new challenges}",
    eprint = "2106.13885",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1140/epjp/s13360-021-02154-9",
    journal = "Eur. Phys. J. Plus",
    volume = "137",
    number = "1",
    pages = "92",
    year = "2022"
}


@article{Freitas:2019bre,
    author = "Freitas, A. and others",
    title = "{Theoretical uncertainties for electroweak and Higgs-boson precision measurements at FCC-ee}",
    eprint = "1906.05379",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IFT-UAM/CSIC-18-021, TUM-HEP-1185/19, KW 19-001, TTK-19-20, UWThPh
  2019-16, UWThPh 2019-16, IFJPAN-IV-2019-8, FR-PHENO-2019-010, DESY 19-105, DESY-19-105",
    month = "6",
    year = "2019"
}


@inproceedings{Accardi:2022oog,
    author = "Accardi, A. and others",
    title = "{Opportunities for precision QCD physics in hadronization at Belle II -- a snowmass whitepaper}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2204.02280",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "4",
    year = "2022"
}


@article{AbdulKhalek:2021gbh,
    author = "Abdul Khalek, R. and others",
    title = "{Science Requirements and Detector Concepts for the Electron-Ion Collider: EIC Yellow Report}",
    eprint = "2103.05419",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "BNL-220990-2021-FORE, JLAB-PHY-21-3198, LA-UR-21-20953",
    month = "3",
    year = "2021"
}


@article{Thomson:2015jda,
    author = "Thomson, Mark",
    title = "{Model-independent measurement of the e$^{{+}}$ e$^{-}$ $\rightarrow $ HZ cross section at a future e$^{{+}}$ e$^{-}$ linear collider using hadronic Z decays}",
    eprint = "1509.02853",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CH-HEP-2015-07",
    doi = "10.1140/epjc/s10052-016-3911-5",
    journal = "Eur. Phys. J. C",
    volume = "76",
    number = "2",
    pages = "72",
    year = "2016"
}


@article{Lai:2021rko,
    author = "Lai, Pei-Zhu and Ruan, Manqi and Kuo, Chia-Ming",
    title = "{Jet performance at the circular electron-positron collider}",
    eprint = "2104.05029",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1088/1748-0221/16/07/P07037",
    journal = "JINST",
    volume = "16",
    number = "07",
    pages = "P07037",
    year = "2021"
}


@article{Boronat:2016tgd,
    author = "Boronat, M. and Fuster, J. and Garcia, I. and Roloff, Ph. and Simoniello, R. and Vos, M.",
    title = "{Jet reconstruction at high-energy electron\textendash{}positron colliders}",
    eprint = "1607.05039",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CLICDP-PUB-2017-002",
    doi = "10.1140/epjc/s10052-018-5594-6",
    journal = "Eur. Phys. J. C",
    volume = "78",
    number = "2",
    pages = "144",
    year = "2018"
}


@article{Larkoski:2017jix,
    author = "Larkoski, Andrew J. and Moult, Ian and Nachman, Benjamin",
    title = "{Jet Substructure at the Large Hadron Collider: A Review of Recent Advances in Theory and Machine Learning}",
    eprint = "1709.04464",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physrep.2019.11.001",
    journal = "Phys. Rept.",
    volume = "841",
    pages = "1--63",
    year = "2020"
}


@book{Marzani:2019hun,
    author = "Marzani, Simone and Soyez, Gregory and Spannowsky, Michael",
    title = "{Looking inside jets: an introduction to jet substructure and boosted-object phenomenology}",
    eprint = "1901.10342",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/978-3-030-15709-8",
    publisher = "Springer",
    volume = "958",
    year = "2019"
}


@article{Abbate:2010xh,
    author = "Abbate, Riccardo and Fickinger, Michael and Hoang, Andre H. and Mateu, Vicent and Stewart, Iain W.",
    title = "{Thrust at $N^{3}LL$ with Power Corrections and a Precision Global Fit for $\alpha_{s}(mZ)$}",
    eprint = "1006.3080",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4101, MPP-2010-7",
    doi = "10.1103/PhysRevD.83.074021",
    journal = "Phys. Rev. D",
    volume = "83",
    pages = "074021",
    year = "2011"
}


@article{Hoang:2015hka,
    author = "Hoang, Andr\'e H. and Kolodrubetz, Daniel W. and Mateu, Vicent and Stewart, Iain W.",
    title = "{Precise determination of $\alpha_s$ from the $C$-parameter distribution}",
    eprint = "1501.04111",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UWTHPH-2015-1, MIT-CTP-4630, LPN14-128",
    doi = "10.1103/PhysRevD.91.094018",
    journal = "Phys. Rev. D",
    volume = "91",
    number = "9",
    pages = "094018",
    year = "2015"
}


@article{Gao:2019mlt,
    author = "Gao, Jun and Gong, Yinqiang and Ju, Wan-Li and Yang, Li Lin",
    title = "{Thrust distribution in Higgs decays at the next-to-leading order and beyond}",
    eprint = "1901.02253",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP03(2019)030",
    journal = "JHEP",
    volume = "03",
    pages = "030",
    year = "2019"
}


@article{ILD:2019kmq,
    author = "Abramowicz, Halina and others",
    collaboration = "ILD",
    title = "{The ILD detector at the ILC}",
    eprint = "1912.04601",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "DESY-19-215",
    month = "12",
    year = "2019"
}


@article{Breidenbach:2021sdo,
    author = "Breidenbach, M. and Brau, J. E. and Burrows, P. and Markiewicz, T. and Stanitzki, M. and Strube, J. and White, A. P.",
    title = "{Updating the SiD Detector concept}",
    eprint = "2110.09965",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "10",
    year = "2021"
}


@article{CLICdp:2018vnx,
    author = "Arominski, Dominik and others",
    collaboration = "CLICdp",
    title = "{A detector for CLIC: main parameters and performance}",
    eprint = "1812.07337",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CLICdp-Note-2018-005",
    month = "12",
    year = "2018"
}


@article{Bacchetta:2019fmz,
    author = "Bacchetta, N. and others",
    title = "{CLD -- A Detector Concept for the FCC-ee}",
    eprint = "1911.12230",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "LCD-Note-2019-001",
    month = "11",
    year = "2019"
}


@article{CALICE:2012eac,
    author = "Adloff, C. and others",
    collaboration = "CALICE",
    title = "{Hadronic energy resolution of a highly granular scintillator-steel hadron calorimeter using software compensation techniques}",
    eprint = "1207.4210",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "MPP-2012-116, CALICE-PUB-2012-002",
    doi = "10.1088/1748-0221/7/09/P09017",
    journal = "JINST",
    volume = "7",
    pages = "P09017",
    year = "2012"
}


@article{Strom:2020wrm,
    author = {Str\"om, R. and Roloff, P.},
    title = "{Physics potential for boosted topologies in top-quark pair production at a multi-TeV Compact Linear Collider}",
    eprint = "2008.05526",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CLICdp-Note-2020-004",
    month = "8",
    year = "2020"
}


@article{Boronat:2014hva,
    author = "Boronat, Mar\c{c}a and Fuster, J. and Garcia, Ignacio and Ros, E. and Vos, Marcel",
    title = "{A robust jet reconstruction algorithm for high-energy lepton colliders}",
    eprint = "1404.4294",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1016/j.physletb.2015.08.055",
    journal = "Phys. Lett. B",
    volume = "750",
    pages = "95--99",
    year = "2015"
}


@article{Stewart:2015waa,
    author = "Stewart, Iain W. and Tackmann, Frank J. and Thaler, Jesse and Vermilion, Christopher K. and Wilkason, Thomas F.",
    title = "{XCone: N-jettiness as an Exclusive Cone Jet Algorithm}",
    eprint = "1508.01516",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4674, DESY-15-087",
    doi = "10.1007/JHEP11(2015)072",
    journal = "JHEP",
    volume = "11",
    pages = "072",
    year = "2015"
}


@article{Collamati:2021sbv,
    author = "Collamati, Francesco and Curatolo, Camilla and Lucchesi, Donatella and Mereghetti, Alessio and Mokhov, Nikolai and Palmer, Mark and Sala, Paola",
    title = "{Advanced assessment of beam-induced background at a muon collider}",
    eprint = "2105.09116",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "FERMILAB-PUB-21-345-AD
",
    doi = "10.1088/1748-0221/16/11/P11009",
    journal = "JINST",
    volume = "16",
    number = "11",
    pages = "P11009",
    year = "2021"
}


@article{Ally:2022rgk,
    author = "Ally, D. and Carpenter, L. and Holmes, T. and Lee, L. and Wagenknecht, P.",
    title = "{Strategies for Beam-Induced Background Reduction at Muon Colliders}",
    eprint = "2203.06773",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "3",
    year = "2022"
}


@inproceedings{MuonCollider:2022ded,
    author = "Bartosik, Nazar and others",
    collaboration = "Muon Collider",
    title = "{Simulated Detector Performance at the Muon Collider}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07964",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "3",
    year = "2022"
}


@article{Thaler:2010tr,
    author = "Thaler, Jesse and Van Tilburg, Ken",
    title = "{Identifying Boosted Objects with N-subjettiness}",
    eprint = "1011.2268",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4191",
    doi = "10.1007/JHEP03(2011)015",
    journal = "JHEP",
    volume = "03",
    pages = "015",
    year = "2011"
}


@article{Thaler:2011gf,
    author = "Thaler, Jesse and Van Tilburg, Ken",
    title = "{Maximizing Boosted Top Identification by Minimizing N-subjettiness}",
    eprint = "1108.2701",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4287",
    doi = "10.1007/JHEP02(2012)093",
    journal = "JHEP",
    volume = "02",
    pages = "093",
    year = "2012"
}


@article{Larkoski:2014gra,
    author = "Larkoski, Andrew J. and Moult, Ian and Neill, Duff",
    title = "{Power Counting to Better Jet Observables}",
    eprint = "1409.6298",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT--CTP-4588",
    doi = "10.1007/JHEP12(2014)009",
    journal = "JHEP",
    volume = "12",
    pages = "009",
    year = "2014"
}


@article{Anderle:2021wcy,
    author = "Anderle, Daniele P. and others",
    title = "{Electron-ion collider in China}",
    eprint = "2102.09222",
    archivePrefix = "arXiv",
    primaryClass = "nucl-ex",
    reportNumber = "Frontiers of Physics, Volume 16 Issue (6):64701, 2021",
    doi = "10.1007/s11467-021-1062-0",
    journal = "Front. Phys. (Beijing)",
    volume = "16",
    number = "6",
    pages = "64701",
    year = "2021"
}


@article{Jacob:1984vnf,
    editor = "Jacob, M.",
    title = "{Proceedings, ECFA-CERN Workshop on large hadron collider in the LEP tunnel}: {Lausanne and Geneva, Switzerland, March 21-27 March, 1984}",
    reportNumber = "CERN-84-10-V-2, CERN-84-10-V-1, ECFA-84-85, CERN-YELLOW-84-10-V-1",
    doi = "10.5170/CERN-1984-010-V-2",
    month = "9",
    year = "1984"
}


@article{LHeCStudyGroup:2012zhm,
    author = "Abelleira Fernandez, J. L. and others",
    collaboration = "LHeC Study Group",
    title = "{A Large Hadron Electron Collider at CERN: Report on the Physics and Design Concepts for Machine and Detector}",
    eprint = "1206.2913",
    archivePrefix = "arXiv",
    primaryClass = "physics.acc-ph",
    reportNumber = "SLAC-R-999, CERN-OPEN-2012-015, LHEC-NOTE-2012-001-GEN",
    doi = "10.1088/0954-3899/39/7/075001",
    journal = "J. Phys. G",
    volume = "39",
    pages = "075001",
    year = "2012"
}


@article{LHeC:2020van,
    author = "Agostini, P. and others",
    collaboration = "LHeC, FCC-he Study Group",
    title = "{The Large Hadron-Electron Collider at the HL-LHC}",
    eprint = "2007.14491",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-ACC-Note-2020-0002, JLAB-ACP-20-3180",
    doi = "10.1088/1361-6471/abf3ba",
    journal = "J. Phys. G",
    volume = "48",
    number = "11",
    pages = "110501",
    year = "2021"
}


@article{Andre:2022xeh,
    author = "Andr\'e, K. D. J. and others",
    title = "{An experiment for electron-hadron scattering at the LHC}",
    eprint = "2201.02436",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1140/epjc/s10052-021-09967-z",
    journal = "Eur. Phys. J. C",
    volume = "82",
    number = "1",
    pages = "40",
    year = "2022"
}


@inproceedings{Acosta:2022ejc,
    author = "Acosta, Darin and Barberis, Emanuela and Hurley, Nicholas and Li, Wei and Colin, Osvaldo Miguel and Wood, Darien and Zuo, Xunwu",
    title = "{The Potential of a TeV-Scale Muon-Ion Collider}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.06258",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "3",
    year = "2022"
}


@article{ATLAS-CONF-2016-035,
    collaboration = "ATLAS",
    title = "{Jet mass reconstruction with the ATLAS Detector in early Run 2 data}",
    reportNumber = "ATLAS-CONF-2016-035, ATLAS-CONF-2016-035",
    month = "7",
    year = "2016"
}


@article{Aleksa:2019pvl,
    author = "Aleksa, M. and others",
    title = "{Calorimeters for the FCC-hh}",
    eprint = "1912.09962",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CERN-FCC-PHYS-2019-0003",
    month = "12",
    year = "2019"
}


@article{GEANT4:2002zbu,
    author = "Agostinelli, S. and others",
    collaboration = "GEANT4",
    title = "{GEANT4--a simulation toolkit}",
    reportNumber = "SLAC-PUB-9350, FERMILAB-PUB-03-339, CERN-IT-2002-003",
    doi = "10.1016/S0168-9002(03)01368-8",
    journal = "Nucl. Instrum. Meth. A",
    volume = "506",
    pages = "250--303",
    year = "2003"
}


@article{CALICE:2019vza,
    author = "Eigen, G. and others",
    collaboration = "CALICE",
    title = "{Characterisation of different stages of hadronic showers using the CALICE Si-W ECAL physics prototype}",
    eprint = "1902.06161",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CALICE-PUB-2019-002",
    doi = "10.1016/j.nima.2019.04.111",
    journal = "Nucl. Instrum. Meth. A",
    volume = "937",
    pages = "41--52",
    year = "2019"
}


@article{dEnterria:2022hzv,
    author = "d'Enterria, D. and others",
    title = "{The strong coupling constant: State of the art and the decade ahead}",
    eprint = "2203.08271",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-22-148-T",
    month = "3",
    year = "2022"
}


@inproceedings{Campbell:2013qaa,
    author = "Campbell, J. M. and others",
    title = "{Working Group Report: Quantum Chromodynamics}",
    booktitle = "{Community Summer Study 2013}: {Snowmass on the Mississippi}",
    eprint = "1310.5189",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ANL-HEP-CP-13-48, FERMILAB-FN-0967-CMS-T",
    month = "10",
    year = "2013"
}


@article{Hou:2022sdf,
    author = "Hou, Tie-Jiun and Lin, Huey-Wen and Yan, Mengshi and Yuan, C. -P.",
    title = "{Impact of lattice $s(x)-\bar{s}(x)$ data in the CTEQ-TEA global analysis}",
    eprint = "2204.07944",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "4",
    year = "2022"
}


@article{Barry:2022itu,
    author = "Barry, P. C. and others",
    title = "{Complementarity of experimental and lattice QCD data on pion parton distributions}",
    eprint = "2204.00543",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "JLAB-THY-22-3592",
    month = "4",
    year = "2022"
}


@article{Bauer:2017ris,
    author = "Bauer, Martin and Neubert, Matthias and Thamm, Andrea",
    title = "{Collider Probes of Axion-Like Particles}",
    eprint = "1708.00443",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP-17-047",
    doi = "10.1007/JHEP12(2017)044",
    journal = "JHEP",
    volume = "12",
    pages = "044",
    year = "2017"
}


@article{ATL-PHYS-PUB-2018-018,
    collaboration = "ATLAS",
    title = "{Prospects for Measurements of Photon-Induced Processes in Ultra-Peripheral Collisions of Heavy Ions with the ATLAS Detector in the LHC Runs 3 and 4}",
    reportNumber = "ATL-PHYS-PUB-2018-018",
    year = "2018"
}


@article{CMS-FSQ-16-012,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Evidence for light-by-light scattering and searches for axion-like particles in ultraperipheral PbPb collisions at $\sqrt{s_\mathrm{NN}} =$ 5.02 TeV}",
    eprint = "1810.04602",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-FSQ-16-012, CERN-EP-2018-271",
    doi = "10.1016/j.physletb.2019.134826",
    journal = "Phys. Lett. B",
    volume = "797",
    pages = "134826",
    year = "2019"
}


@article{Adamova:2019vkf,
    author = "Adamov\'a, D. and others",
    title = "{A next-generation LHC heavy-ion experiment}",
    eprint = "1902.01211",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "1",
    year = "2019"
}


@inproceedings{dEnterria:2022sut,
    author = "d'Enterria, David and others",
    title = "{Opportunities for new physics searches with heavy ions at colliders}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.05939",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@article{Chen:2022msz,
    author = "Chen, Siyu and Glioti, Alfredo and Rattazzi, Riccardo and Ricci, Lorenzo and Wulzer, Andrea",
    title = "{Learning from radiation at a very high energy lepton collider}",
    eprint = "2202.10509",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2022)180",
    journal = "JHEP",
    volume = "05",
    pages = "180",
    year = "2022"
}


@article{Buttazzo:2020uzc,
    author = "Buttazzo, Dario and Franceschini, Roberto and Wulzer, Andrea",
    title = "{Two Paths Towards Precision at a Very High Energy Lepton Collider}",
    eprint = "2012.11555",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-216",
    doi = "10.1007/JHEP05(2021)219",
    journal = "JHEP",
    volume = "05",
    pages = "219",
    year = "2021"
}


@article{Thamm:2015zwa,
    author = "Thamm, Andrea and Torre, Riccardo and Wulzer, Andrea",
    title = "{Future tests of Higgs compositeness: direct vs indirect}",
    eprint = "1502.01701",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DFPD-2014-TH-03, MITP-14-109",
    doi = "10.1007/JHEP07(2015)100",
    journal = "JHEP",
    volume = "07",
    pages = "100",
    year = "2015"
}


@article{FCC:2018byv,
    author = "Abada, A. and others",
    collaboration = "FCC",
    title = "{FCC Physics Opportunities}: {Future Circular Collider Conceptual Design Report Volume 1}",
    reportNumber = "CERN-ACC-2018-0056",
    doi = "10.1140/epjc/s10052-019-6904-3",
    journal = "Eur. Phys. J. C",
    volume = "79",
    number = "6",
    pages = "474",
    year = "2019"
}


@inproceedings{Lane:2022ybv,
    author = "Lane, Kenneth",
    title = "{The Composite Higgs Signal at the Next Big Collider}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.03710",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@article{Draper:2016pys,
    author = "Draper, Patrick and Rzehak, Heidi",
    title = "{A Review of Higgs Mass Calculations in Supersymmetric Models}",
    eprint = "1601.01890",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DIAS-2016-1, FR-PHENO-2016-001, CP3-ORIGINS-2016-001-DNRF90",
    doi = "10.1016/j.physrep.2016.01.001",
    journal = "Phys. Rept.",
    volume = "619",
    pages = "1--24",
    year = "2016"
}


@article{ATLAS:2022hsp,
    collaboration = "ATLAS",
    title = "{Snowmass White Paper Contribution: Physics with the Phase-2 ATLAS and CMS Detectors}",
    reportNumber = "ATL-PHYS-PUB-2022-018",
    year = "2022"
}


@article{Dobrescu:2013cmh,
    author = "Dobrescu, Bogdan A. and Yu, Felix",
    title = "{Coupling-Mass Mapping of Dijet Peak Searches}",
    eprint = "1306.2629",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-13-185-T",
    doi = "10.1103/PhysRevD.88.035021",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "3",
    pages = "035021",
    year = "2013",
    note = "[Erratum: Phys.Rev.D 90, 079901 (2014)]"
}


@article{Dobrescu:2021vak,
    author = "Dobrescu, Bogdan A. and Yu, Felix",
    title = "{Dijet and electroweak limits on a $Z'$ boson coupled to quarks}",
    eprint = "2112.05392",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP-17-048, FERMILAB-PUB-21-698-T",
    month = "12",
    year = "2021"
}


@article{Aime:2022flm,
    author = "Aime, Chiara and others",
    title = "{Muon Collider Physics Summary}",
    eprint = "2203.07256",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-22-377-PPD",
    month = "3",
    year = "2022"
}


@article{Helsens:2019bfw,
    author = "Helsens, Clement and Jamin, David and Mangano, Michelangelo L. and Rizzo, Thomas G. and Selvaggi, Michele",
    title = "{Heavy resonances at energy-frontier hadron colliders}",
    eprint = "1902.11217",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2019-020, SLAC-PUB-17408",
    doi = "10.1140/epjc/s10052-019-7062-3",
    journal = "Eur. Phys. J. C",
    volume = "79",
    pages = "569",
    year = "2019"
}


@article{ATL-PHYS-PUB-2018-044,
    collaboration = "ATLAS",
    title = "{Prospects for searches for heavy $Z^\prime$ and $W^\prime$ bosons in fermionic final states with the ATLAS experiment at the HL-LHC}",
    reportNumber = "ATL-PHYS-PUB-2018-044",
    year = "2018"
}


@article{CMS-PAS-FTR-21-005,
    collaboration = "CMS",
    title = "{Sensitivity projections for a search for new phenomena at high dilepton mass for the LHC Run 3 and the HL-LHC}",
    reportNumber = "CMS-PAS-FTR-21-005",
    year = "2022"
}


@inproceedings{Suehara:2022pwv,
    author = "Suehara, Taikan",
    title = "{Two-fermion final states at International Linear Collider}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07272",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}


@inproceedings{Han:2022mzp,
    author = "Han, Tao and Li, Tong and Wang, Xing",
    title = "{Axion-Like Particles at High Energy Muon Colliders -- A White paper for Snowmass 2021}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.05484",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-2202",
    month = "3",
    year = "2022"
}


@article{Guler:2022czi,
    author = "Gurpinar Guler, Emine and Guler, Yalcin and Harris, Robert M.",
    title = "{Mass distributions of dijet resonances from excited quarks at proton-proton colliders}",
    eprint = "2205.02781",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-22-301-PPD-SCD",
    month = "5",
    year = "2022"
}


@article{Thomas:1998wy,
    author = "Thomas, Scott D. and Wells, James D.",
    title = "{Phenomenology of Massive Vectorlike Doublet Leptons}",
    eprint = "hep-ph/9804359",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-7799, SU-ITP-98-22",
    doi = "10.1103/PhysRevLett.81.34",
    journal = "Phys. Rev. Lett.",
    volume = "81",
    pages = "34--37",
    year = "1998"
}


@article{Capdevilla:2021fmj,
    author = "Capdevilla, Rodolfo and Meloni, Federico and Simoniello, Rosa and Zurita, Jose",
    title = "{Hunting wino and higgsino dark matter at the muon collider with disappearing tracks}",
    eprint = "2102.11292",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-21-019, DESY 21-019, IFIC/21-03",
    doi = "10.1007/JHEP06(2021)133",
    journal = "JHEP",
    volume = "06",
    pages = "133",
    year = "2021"
}


@article{Han:2018wus,
    author = "Han, Tao and Mukhopadhyay, Satyanarayan and Wang, Xing",
    title = "{Electroweak Dark Matter at Future Hadron Colliders}",
    eprint = "1805.00015",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-1806",
    doi = "10.1103/PhysRevD.98.035026",
    journal = "Phys. Rev. D",
    volume = "98",
    number = "3",
    pages = "035026",
    year = "2018"
}


@inproceedings{PardodeVera:2020zlr,
    author = "Pardo de Vera, Mar\'\i{}a Teresa N\'u\~nez and Berggren, Mikael and List, Jenny",
    title = "{Chargino production at the ILC}",
    booktitle = "{International Workshop on Future Linear Colliders}",
    eprint = "2002.01239",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "2",
    year = "2020"
}


@article{Curtin:2017bxr,
    author = "Curtin, David and Deshpande, Kaustubh and Fischer, Oliver and Zurita, Jos\'e",
    title = "{New Physics Opportunities for Long-Lived Particles at Electron-Proton Colliders}",
    eprint = "1712.07135",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TTP17-053",
    doi = "10.1007/JHEP07(2018)024",
    journal = "JHEP",
    volume = "07",
    pages = "024",
    year = "2018"
}


@article{Saito:2019rtg,
    author = "Saito, Masahiko and Sawada, Ryu and Terashi, Koji and Asai, Shoji",
    title = "{Discovery reach for wino and higgsino dark matter with a disappearing track signature at a 100 TeV $pp$ collider}",
    eprint = "1901.02987",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-019-6974-2",
    journal = "Eur. Phys. J. C",
    volume = "79",
    number = "6",
    pages = "469",
    year = "2019"
}


@article{Rinchiuso:2020skh,
    author = "Rinchiuso, Lucia and Macias, Oscar and Moulin, Emmanuel and Rodd, Nicholas L. and Slatyer, Tracy R.",
    title = "{Prospects for detecting heavy WIMP dark matter with the Cherenkov Telescope Array: The Wino and Higgsino}",
    eprint = "2008.00692",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.HE",
    reportNumber = "MIT-CTP 5120, IRFU-20-13",
    doi = "10.1103/PhysRevD.103.023011",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "2",
    pages = "023011",
    year = "2021"
}


@article{Alimena:2022hfr,
    author = "Alimena, J. and others",
    title = "{Searches for Long-Lived Particles at the Future FCC-ee}",
    eprint = "2203.05502",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "3",
    year = "2022"
}


@article{Cirelli:2005uq,
    author = "Cirelli, Marco and Fornengo, Nicolao and Strumia, Alessandro",
    title = "{Minimal dark matter}",
    eprint = "hep-ph/0512090",
    archivePrefix = "arXiv",
    reportNumber = "DFTT40-2005, IFUP-TH-2005-34",
    doi = "10.1016/j.nuclphysb.2006.07.012",
    journal = "Nucl. Phys. B",
    volume = "753",
    pages = "178--194",
    year = "2006"
}


@article{Cirelli:2009uv,
    author = "Cirelli, Marco and Strumia, Alessandro",
    title = "{Minimal Dark Matter: Model and results}",
    eprint = "0903.3381",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IFUP-TH-2009-04, SACLAY-T09-010",
    doi = "10.1088/1367-2630/11/10/105005",
    journal = "New J. Phys.",
    volume = "11",
    pages = "105005",
    year = "2009"
}


@article{Planck:2018vyg,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020",
    note = "[Erratum: Astron.Astrophys. 652, C4 (2021)]"
}


@article{Belotsky:2005dk,
    author = "Belotsky, Konstantin M. and Khlopov, M. Yu. and Legonkov, S. V. and Shibaev, K. I.",
    editor = "Alimi, J. M. and Khlopov, M. Yu. and Melnikov, V. N.",
    title = "{Effects of new long-range interaction: Recombination of relic heavy neutrinos and antineutrinos}",
    eprint = "astro-ph/0504621",
    archivePrefix = "arXiv",
    journal = "Grav. Cosmol.",
    volume = "11",
    pages = "27--33",
    year = "2005"
}


@article{Hisano:2006nn,
    author = "Hisano, Junji and Matsumoto, Shigeki and Nagai, Minoru and Saito, Osamu and Senami, Masato",
    title = "{Non-perturbative effect on thermal relic abundance of dark matter}",
    eprint = "hep-ph/0610249",
    archivePrefix = "arXiv",
    reportNumber = "KEK-TH-1111",
    doi = "10.1016/j.physletb.2007.01.012",
    journal = "Phys. Lett. B",
    volume = "646",
    pages = "34--38",
    year = "2007"
}


@article{Cirelli:2007xd,
    author = "Cirelli, Marco and Strumia, Alessandro and Tamburini, Matteo",
    title = "{Cosmology and Astrophysics of Minimal Dark Matter}",
    eprint = "0706.4071",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IFUP-TH-2007-12, SACLAY-T07-052",
    doi = "10.1016/j.nuclphysb.2007.07.023",
    journal = "Nucl. Phys. B",
    volume = "787",
    pages = "152--175",
    year = "2007"
}


@article{An:2016gad,
    author = "An, Haipeng and Wise, Mark B. and Zhang, Yue",
    title = "{Effects of Bound States on Dark Matter Annihilation}",
    eprint = "1604.01776",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CALT-TH-2016-005",
    doi = "10.1103/PhysRevD.93.115020",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "11",
    pages = "115020",
    year = "2016"
}


@article{Mitridate:2017izz,
    author = "Mitridate, Andrea and Redi, Michele and Smirnov, Juri and Strumia, Alessandro",
    title = "{Cosmological Implications of Dark Matter Bound States}",
    eprint = "1702.01141",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2017-030, IFUP-TH-2017",
    doi = "10.1088/1475-7516/2017/05/006",
    journal = "JCAP",
    volume = "05",
    pages = "006",
    year = "2017"
}


@article{DelNobile:2015bqo,
    author = "Del Nobile, Eugenio and Nardecchia, Marco and Panci, Paolo",
    title = "{Millicharge or Decay: A Critical Take on Minimal Dark Matter}",
    eprint = "1512.05353",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DFPD-2015-TH-29",
    doi = "10.1088/1475-7516/2016/04/048",
    journal = "JCAP",
    volume = "04",
    pages = "048",
    year = "2016"
}


@article{Strategy:2019vxc,
    author = "Ellis, Richard Keith and others",
    title = "{Physics Briefing Book}: {Input for the European Strategy for Particle Physics Update 2020}",
    eprint = "1910.11775",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-ESU-004",
    month = "10",
    year = "2019"
}


@article{Han:2020uak,
    author = "Han, Tao and Liu, Zhen and Wang, Lian-Tao and Wang, Xing",
    title = "{WIMPs at High Energy Muon Colliders}",
    eprint = "2009.11287",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC 2009",
    doi = "10.1103/PhysRevD.103.075004",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "7",
    pages = "075004",
    year = "2021"
}


@inproceedings{Han:2022ubw,
    author = "Han, Tao and Liu, Zhen and Wang, Lian-Tao and Wang, Xing",
    title = "{WIMP Dark Matter at High Energy Muon Colliders $-$A White Paper for Snowmass 2021}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.07351",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-2201",
    month = "3",
    year = "2022"
}


@article{Bottaro:2021srh,
    author = "Bottaro, Salvatore and Strumia, Alessandro and Vignaroli, Natascia",
    title = "{Minimal Dark Matter bound states at future colliders}",
    eprint = "2103.12766",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP06(2021)143",
    journal = "JHEP",
    volume = "06",
    pages = "143",
    year = "2021"
}


@article{Bottaro:2021snn,
    author = "Bottaro, Salvatore and Buttazzo, Dario and Costa, Marco and Franceschini, Roberto and Panci, Paolo and Redigolo, Diego and Vittorio, Ludovico",
    title = "{Closing the window on WIMP Dark Matter}",
    eprint = "2107.09688",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-021-09917-9",
    journal = "Eur. Phys. J. C",
    volume = "82",
    number = "1",
    pages = "31",
    year = "2022"
}


@article{Bottaro:2022one,
    author = "Bottaro, Salvatore and Buttazzo, Dario and Costa, Marco and Franceschini, Roberto and Panci, Paolo and Redigolo, Diego and Vittorio, Ludovico",
    title = "{The last Complex WIMPs standing}",
    eprint = "2205.04486",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2022-080",
    month = "5",
    year = "2022"
}


@inproceedings{Black:2022qlg,
    author = "Black, Kevin and Bose, Tulika and Chen, Yuze and Dasu, Sridhara and Jia, Haoyi and Pinna, Deborah and Sharma, Varun and Venkatasubramanian, Nikhilesh and Vuosalo, Carl",
    title = "{Prospects for Heavy WIMP Dark Matter Searches at Muon Colliders}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2205.10404",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "5",
    year = "2022"
}


@article{Abercrombie:2015wmb,
    author = "Abercrombie, Daniel and others",
    editor = "Boveia, Antonio and Doglioni, Caterina and Lowette, Steven and Malik, Sarah and Mrenna, Stephen",
    title = "{Dark Matter benchmark models for early LHC Run-2 Searches: Report of the ATLAS/CMS Dark Matter Forum}",
    eprint = "1507.00966",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-PUB-15-282-CD",
    doi = "10.1016/j.dark.2019.100371",
    journal = "Phys. Dark Univ.",
    volume = "27",
    pages = "100371",
    year = "2020"
}


@article{Batell:2018fqo,
    author = "Batell, Brian and Freitas, Ayres and Ismail, Ahmed and Mckeen, David",
    title = "{Probing Light Dark Matter with a Hadrophilic Scalar Mediator}",
    eprint = "1812.05103",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-1817",
    doi = "10.1103/PhysRevD.100.095020",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "9",
    pages = "095020",
    year = "2019"
}


@article{Batell:2021xsi,
    author = "Batell, Brian and Freitas, Ayres and Ismail, Ahmed and McKeen, David and Rai, Mudit",
    title = "{Renormalizable models of flavor-specific scalars}",
    eprint = "2107.08059",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-2114",
    doi = "10.1103/PhysRevD.104.115032",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "11",
    pages = "115032",
    year = "2021"
}


@inproceedings{Rizzo:2022qan,
    author = "Rizzo, Thomas G.",
    title = "{Portal Matter and Dark Sector Phenomenology at Colliders}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2202.02222",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SLAC-PUB-17633",
    month = "2",
    year = "2022"
}


@article{Strassler:2006im,
    author = "Strassler, Matthew J. and Zurek, Kathryn M.",
    title = "{Echoes of a hidden valley at hadron colliders}",
    eprint = "hep-ph/0604261",
    archivePrefix = "arXiv",
    doi = "10.1016/j.physletb.2007.06.055",
    journal = "Phys. Lett. B",
    volume = "651",
    pages = "374--379",
    year = "2007"
}


@article{Bai:2013xga,
    author = "Bai, Yang and Schwaller, Pedro",
    title = "{Scale of dark QCD}",
    eprint = "1306.4676",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.89.063522",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "6",
    pages = "063522",
    year = "2014"
}


@article{Bernreuther:2019pfb,
    author = {Bernreuther, Elias and Kahlhoefer, Felix and Kr\"amer, Michael and Tunney, Patrick},
    title = "{Strongly interacting dark sectors in the early Universe and at the LHC through a simplified portal}",
    eprint = "1907.04346",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TTK-19-25, P3H-19-019",
    doi = "10.1007/JHEP01(2020)162",
    journal = "JHEP",
    volume = "01",
    pages = "162",
    year = "2020"
}


@article{Cline:2016nab,
    author = "Cline, James M. and Huang, Weicong and Moore, Guy D.",
    title = "{Challenges for models with composite states}",
    eprint = "1607.07865",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.94.055029",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "5",
    pages = "055029",
    year = "2016"
}


@article{Mies:2020mzw,
    author = "Mies, Hanna and Scherb, Christiane and Schwaller, Pedro",
    title = "{Collider constraints on dark mediators}",
    eprint = "2011.13990",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP/20-068,P3H-20-069,TTK-20-41",
    doi = "10.1007/JHEP04(2021)049",
    journal = "JHEP",
    volume = "04",
    pages = "049",
    year = "2021"
}


@article{Asadi:2021yml,
    author = "Asadi, Pouya and Kramer, Eric David and Kuflik, Eric and Ridgway, Gregory W. and Slatyer, Tracy R. and Smirnov, Juri",
    title = "{Accidentally Asymmetric Dark Matter}",
    eprint = "2103.09822",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP/5284",
    doi = "10.1103/PhysRevLett.127.211101",
    journal = "Phys. Rev. Lett.",
    volume = "127",
    number = "21",
    pages = "211101",
    year = "2021"
}


@article{Kulkarni:2022bvh,
    author = "Kulkarni, Suchita and Maas, Axel and Mee, Se\'an and Nikolic, Marco and Pradler, Josef and Zierler, Fabian",
    title = "{Low-energy effective description of dark $Sp(4)$ theories}",
    eprint = "2202.05191",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "2",
    year = "2022"
}


@article{Feng:2022inv,
    author = "Feng, Jonathan L. and others",
    title = "{The Forward Physics Facility at the High-Luminosity LHC}",
    eprint = "2203.05090",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2022-01, CERN-PBC-Notes-2022-001,
  FERMILAB-PUB-22-094-ND-SCD-T, INT-PUB-22-006, BONN-TH-2022-04",
    month = "3",
    year = "2022"
}


@article{Abdesselam:2010pt,
    author = "Abdesselam, A. and others",
    title = "{Boosted Objects: A Probe of Beyond the Standard Model Physics}",
    eprint = "1012.5412",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SLAC-PUB-15081, FERMILAB-PUB-10-617-CMS",
    doi = "10.1140/epjc/s10052-011-1661-y",
    journal = "Eur. Phys. J. C",
    volume = "71",
    pages = "1661",
    year = "2011"
}


@article{Altheimer:2012mn,
    author = "Altheimer, A. and others",
    title = "{Jet Substructure at the Tevatron and LHC: New results, new tools, new benchmarks}",
    eprint = "1201.0008",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SLAC-R-990, FERMILAB-PUB-12-897-T",
    doi = "10.1088/0954-3899/39/6/063001",
    journal = "J. Phys. G",
    volume = "39",
    pages = "063001",
    year = "2012"
}


@article{Altheimer:2013yza,
    author = "Altheimer, A. and others",
    title = "{Boosted Objects and Jet Substructure at the LHC. Report of BOOST2012, held at IFIC Valencia, 23rd-27th of July 2012}",
    eprint = "1311.2708",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-PUB-13-669",
    doi = "10.1140/epjc/s10052-014-2792-8",
    journal = "Eur. Phys. J. C",
    volume = "74",
    number = "3",
    pages = "2792",
    year = "2014"
}


@article{Adams:2015hiv,
    author = "Adams, D. and others",
    title = "{Towards an Understanding of the Correlations in Jet Substructure}",
    eprint = "1504.00679",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-15-670-CMS, SLAC-PUB-16703",
    doi = "10.1140/epjc/s10052-015-3587-2",
    journal = "Eur. Phys. J. C",
    volume = "75",
    number = "9",
    pages = "409",
    year = "2015"
}


@article{Kogler:2018hem,
    author = "Kogler, Roman and others",
    title = "{Jet Substructure at the Large Hadron Collider: Experimental Review}",
    eprint = "1803.06991",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "FERMILAB-PUB-18-123-PPD",
    doi = "10.1103/RevModPhys.91.045003",
    journal = "Rev. Mod. Phys.",
    volume = "91",
    number = "4",
    pages = "045003",
    year = "2019"
}


@book{Kogler:2021kkw,
    author = "Kogler, Roman",
    title = "{Advances in Jet Substructure at the LHC: Algorithms, Measurements and Searches for New Physical Phenomena}",
    doi = "10.1007/978-3-030-72858-8",
    isbn = "978-3-030-72857-1, 978-3-030-72858-8",
    publisher = "Springer",
    volume = "284",
    month = "5",
    year = "2021"
}


@article{Yeh:2019xbj,
    author = "Yeh, C. -H. and Chekanov, S. V. and Kotwal, A. V. and Proudfoot, J. and Sen, S. and Tran, N. V. and Yu, S. -S.",
    title = "{Studies of granularity of a hadronic calorimeter for tens-of-TeV jets at a 100 TeV $pp$ collider}",
    eprint = "1901.11146",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "ANL-HEP-149528, FERMILAB-PUB-19-089-PPD",
    doi = "10.1088/1748-0221/14/05/P05008",
    journal = "JINST",
    volume = "14",
    number = "05",
    pages = "P05008",
    year = "2019"
}


@article{Coleman:2017fiq,
    author = "Coleman, Evan and Freytsis, Marat and Hinzmann, Andreas and Narain, Meenakshi and Thaler, Jesse and Tran, Nhan and Vernieri, Caterina",
    title = "{The importance of calorimetry for highly-boosted jet substructure}",
    eprint = "1709.08705",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-17-347-E, MIT-CTP-4935",
    doi = "10.1088/1748-0221/13/01/T01003",
    journal = "JINST",
    volume = "13",
    number = "01",
    pages = "T01003",
    year = "2018"
}


@article{Gras:2017jty,
    author = {Gras, Philippe and H\"oche, Stefan and Kar, Deepak and Larkoski, Andrew and L\"onnblad, Leif and Pl\"atzer, Simon and Si\'odmok, Andrzej and Skands, Peter and Soyez, Gregory and Thaler, Jesse},
    title = "{Systematics of quark/gluon tagging}",
    eprint = "1704.03878",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4885, COEPP-MN-17-2, MCNET-17-04",
    doi = "10.1007/JHEP07(2017)091",
    journal = "JHEP",
    volume = "07",
    pages = "091",
    year = "2017"
}


@proceedings{Proceedings:2018jsb,
    author = "Andersen, J. R. and others",
    title = "{Les Houches 2017: Physics at TeV Colliders Standard Model Working Group Report}",
    eprint = "1803.07977",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-18-122-CD-T, UWTHPH-2018-5",
    month = "3",
    year = "2018"
}


@inproceedings{Amoroso:2020lgh,
    author = "Amoroso, S. and others",
    title = "{Les Houches 2019: Physics at TeV Colliders: Standard Model Working Group Report}",
    booktitle = "{11th Les Houches Workshop on Physics at TeV Colliders}: {PhysTeV Les Houches}",
    eprint = "2003.01700",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2020"
}


@article{CMS:2017wtu,
    author = "Sirunyan, A. M. and others",
    collaboration = "CMS",
    title = "{Identification of heavy-flavour jets with the CMS detector in pp collisions at 13 TeV}",
    eprint = "1712.07158",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "CMS-BTV-16-002, CERN-EP-2017-326",
    doi = "10.1088/1748-0221/13/05/P05011",
    journal = "JINST",
    volume = "13",
    number = "05",
    pages = "P05011",
    year = "2018"
}


@article{ATLAS:2019bwq,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{ATLAS b-jet identification performance and efficiency measurement with $t{\bar{t}}$ events in pp collisions at $\sqrt{s}=13$ TeV}",
    eprint = "1907.05120",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2019-132",
    doi = "10.1140/epjc/s10052-019-7450-8",
    journal = "Eur. Phys. J. C",
    volume = "79",
    number = "11",
    pages = "970",
    year = "2019"
}


@article{CMS:2021scf,
    author = "Tumasyan, Armen and others",
    collaboration = "CMS",
    title = "{A new calibration method for charm jet identification validated with proton-proton collision events at $\sqrt{s}$ =13 TeV}",
    eprint = "2111.03027",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-BTV-20-001, CERN-EP-2021-177",
    doi = "10.1088/1748-0221/17/03/P03014",
    journal = "JINST",
    volume = "17",
    number = "03",
    pages = "P03014",
    year = "2022"
}


@article{ATLAS:2021cxe,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{Measurement of the c-jet mistagging efficiency in $t\bar{t}$~events using pp collision data at $\sqrt{s}=13$~$\text {TeV}$ collected with the ATLAS detector}",
    eprint = "2109.10627",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2021-166",
    doi = "10.1140/epjc/s10052-021-09843-w",
    journal = "Eur. Phys. J. C",
    volume = "82",
    number = "1",
    pages = "95",
    year = "2022"
}


@article{Erdmann:2020ovh,
    author = "Erdmann, Johannes and Nackenhorst, Olaf and Zei\ss{}ner, Sonja Verena",
    title = "{Maximum performance of strange-jet tagging at hadron colliders}",
    eprint = "2011.10736",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1088/1748-0221/16/08/P08039",
    journal = "JINST",
    volume = "16",
    number = "08",
    pages = "P08039",
    year = "2021"
}


@article{Nakai:2020kuu,
    author = "Nakai, Yuichiro and Shih, David and Thomas, Scott",
    title = "{Strange Jet Tagging}",
    eprint = "2003.09517",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2020"
}


@article{Erdmann:2019blf,
    author = "Erdmann, Johannes",
    title = "{A tagger for strange jets based on tracking information using long short-term memory}",
    eprint = "1907.07505",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    doi = "10.1088/1748-0221/15/01/P01021",
    journal = "JINST",
    volume = "15",
    number = "01",
    pages = "P01021",
    year = "2020"
}


@article{Nachman:2022emq,
    author = "Nachman, Ben and others",
    title = "{Jets and Jet Substructure at Future Colliders}",
    eprint = "2203.07462",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-22-186-SCD-T",
    month = "3",
    year = "2022"
}


@article{Chiu:2021sgs,
    author = "Chiu, Wen Han and Liu, Zhen and Low, Matthew and Wang, Lian-Tao",
    title = "{Jet timing}",
    eprint = "2109.01682",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-21-372-T",
    doi = "10.1007/JHEP01(2022)014",
    journal = "JHEP",
    volume = "01",
    pages = "014",
    year = "2022"
}


@article{Chatterjee:2019brg,
    author = "Chatterjee, Suman and Godbole, Rohini and Roy, Tuhin S.",
    title = "{Jets with electrons from boosted top quarks}",
    eprint = "1909.11041",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TIFR/TH/19-33",
    doi = "10.1007/JHEP01(2020)170",
    journal = "JHEP",
    volume = "01",
    pages = "170",
    year = "2020"
}


@article{Mitra:2016kov,
    author = "Mitra, Manimala and Ruiz, Richard and Scott, Darren J. and Spannowsky, Michael",
    title = "{Neutrino Jets from High-Mass $W_R$ Gauge Bosons in TeV-Scale Left-Right Symmetric Models}",
    eprint = "1607.03504",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPPP-16-65, CPT-16-130",
    doi = "10.1103/PhysRevD.94.095016",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "9",
    pages = "095016",
    year = "2016"
}


@article{Nemevsek:2018bbt,
    author = "Nemev\v{s}ek, Miha and Nesti, Fabrizio and Popara, Goran",
    title = "{Keung-Senjanovi\'c process at the LHC: From lepton number violation to displaced vertices to invisible decays}",
    eprint = "1801.05813",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.97.115018",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "11",
    pages = "115018",
    year = "2018"
}


@article{duPlessis:2021xuc,
    author = "du Plessis, K. and Flores, M. M. and Kar, D. and Sinha, S. and van der Schyf, H.",
    title = "{Hitting two BSM particles with one lepton-jet: search for a top partner decaying to a dark photon, resulting in a lepton-jet}",
    eprint = "2112.08425",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "12",
    year = "2021"
}


@article{Dube:2017jgo,
    author = "Dube, Sourabh and Gadkari, Divya and Thalapillil, Arun M.",
    title = "{Lepton-Jets and Low-Mass Sterile Neutrinos at Hadron Colliders}",
    eprint = "1707.00008",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.96.055031",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "5",
    pages = "055031",
    year = "2017"
}


@article{Wang:2021uyb,
    author = "Wang, Daohan and Wu, Lei and Yang, Jin Min and Zhang, Mengchao",
    title = "{Photon-jet events as a probe of axionlike particles at the LHC}",
    eprint = "2102.01532",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.104.095016",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "9",
    pages = "095016",
    year = "2021"
}


@article{Sheff:2020jyw,
    author = "Sheff, Benjamin and Steinberg, Noah and Wells, James D.",
    title = "{Higgs boson decays into narrow diphoton jets and their search strategies at the Large Hadron Collider}",
    eprint = "2008.10568",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.104.036009",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "3",
    pages = "036009",
    year = "2021"
}


@article{Kar:2020bws,
    author = "Kar, Deepak and Sinha, Sukanya",
    title = "{Exploring jet substructure in semi-visible jets}",
    eprint = "2007.11597",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.21468/SciPostPhys.10.4.084",
    journal = "SciPost Phys.",
    volume = "10",
    number = "4",
    pages = "084",
    year = "2021"
}


@article{Canelli:2021aps,
    author = "Canelli, Florencia and de Cosa, Annapaola and Pottier, Luc Le and Niedziela, Jeremi and Pedro, Kevin and Pierini, Maurizio",
    title = "{Autoencoders for semivisible jet detection}",
    eprint = "2112.02864",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP02(2022)074",
    journal = "JHEP",
    volume = "02",
    pages = "074",
    year = "2022"
}


@article{CMS:2021dzb,
    author = "Tumasyan, Armen and others",
    collaboration = "CMS",
    title = "{Search for a right-handed W boson and a heavy neutrino in proton-proton collisions at $ \sqrt{s} $ = 13 TeV}",
    eprint = "2112.03949",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-EXO-20-002, CERN-EP-2021-228",
    doi = "10.1007/JHEP04(2022)047",
    journal = "JHEP",
    volume = "04",
    pages = "047",
    year = "2022"
}


@article{ATLAS:2019isd,
    author = "Aaboud, Morad and others",
    collaboration = "ATLAS",
    title = "{Search for a right-handed gauge boson decaying into a high-momentum heavy neutrino and a charged lepton in $pp$ collisions with the ATLAS detector at $\sqrt{s}=13$ TeV}",
    eprint = "1904.12679",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2019-052",
    doi = "10.1016/j.physletb.2019.134942",
    journal = "Phys. Lett. B",
    volume = "798",
    pages = "134942",
    year = "2019"
}


@article{CMS:2021dzg,
    author = "Tumasyan, Armen and others",
    collaboration = "CMS",
    title = "{Search for resonant production of strongly coupled dark matter in proton-proton collisions at 13 TeV}",
    eprint = "2112.11125",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-EXO-19-020, CERN-EP-2021-252",
    month = "12",
    year = "2021"
}


@article{ATLAS:2019tkk,
    author = "Aad, Georges and others",
    collaboration = "ATLAS",
    title = "{Search for light long-lived neutral particles produced in $pp$ collisions at $\sqrt{s} =$ 13 TeV and decaying into collimated leptons or light hadrons with the ATLAS detector}",
    eprint = "1909.01246",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2019-140",
    doi = "10.1140/epjc/s10052-020-7997-4",
    journal = "Eur. Phys. J. C",
    volume = "80",
    number = "5",
    pages = "450",
    year = "2020"
}


@article{CMS:2019qjk,
    author = "Sirunyan, Albert M and others",
    collaboration = "CMS",
    title = "{Search for long-lived particles using nonprompt jets and missing transverse momentum with proton-proton collisions at $\sqrt{s} =$ 13 TeV}",
    eprint = "1906.06441",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CMS-EXO-19-001, CERN-EP-2019-113",
    doi = "10.1016/j.physletb.2019.134876",
    journal = "Phys. Lett. B",
    volume = "797",
    pages = "134876",
    year = "2019"
}


@article{Chen:2022jhb,
    author = "Chen, Hao and Moult, Ian and Sandor, Joshua and Zhu, Hua Xing",
    title = "{Celestial Blocks and Transverse Spin in the Three-Point Energy Correlator}",
    eprint = "2202.04085",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "2",
    year = "2022"
}


@article{Chen:2021gdk,
    author = "Chen, Hao and Moult, Ian and Zhu, Hua Xing",
    title = "{Spinning Gluons from the QCD Light-Ray OPE}",
    eprint = "2104.00009",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2021"
}


@article{Chen:2020adz,
    author = "Chen, Hao and Moult, Ian and Zhu, Hua Xing",
    title = "{Quantum Interference in Jet Substructure from Spinning Gluons}",
    eprint = "2011.02492",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.126.112003",
    journal = "Phys. Rev. Lett.",
    volume = "126",
    number = "11",
    pages = "112003",
    year = "2021"
}


@article{Chen:2019bpb,
    author = "Chen, Hao and Luo, Ming-Xing and Moult, Ian and Yang, Tong-Zhi and Zhang, Xiaoyuan and Zhu, Hua Xing",
    title = "{Three point energy correlators in the collinear limit: symmetries, dualities and analytic results}",
    eprint = "1912.11050",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP08(2020)028",
    journal = "JHEP",
    volume = "08",
    number = "08",
    pages = "028",
    year = "2020"
}


@article{Chen:2020vvp,
    author = "Chen, Hao and Moult, Ian and Zhang, XiaoYuan and Zhu, Hua Xing",
    title = "{Rethinking jets with energy correlators: Tracks, resummation, and analytic continuation}",
    eprint = "2004.11381",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.102.054012",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "5",
    pages = "054012",
    year = "2020"
}


@article{Holguin:2022epo,
    author = "Holguin, Jack and Moult, Ian and Pathak, Aditya and Procura, Massimiliano",
    title = "{A New Paradigm for Precision Top Physics: Weighing the Top with Energy Correlators}",
    eprint = "2201.08393",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "1",
    year = "2022"
}


@article{Komiske:2022enw,
    author = "Komiske, Patrick T. and Moult, Ian and Thaler, Jesse and Zhu, Hua Xing",
    title = "{Analyzing N-point Energy Correlators Inside Jets with CMS Open Data}",
    eprint = "2201.07800",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP 5389",
    month = "1",
    year = "2022"
}


@article{Kologlu:2019mfz,
    author = "Kologlu, Murat and Kravchuk, Petr and Simmons-Duffin, David and Zhiboedov, Alexander",
    title = "{The light-ray OPE and conformal colliders}",
    eprint = "1905.01311",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CALT-TH 2019-013, CERN-TH-2019-055",
    doi = "10.1007/JHEP01(2021)128",
    journal = "JHEP",
    volume = "01",
    pages = "128",
    year = "2021"
}


@article{Dasgupta:2013ihk,
    author = "Dasgupta, Mrinal and Fregoso, Alessandro and Marzani, Simone and Salam, Gavin P.",
    title = "{Towards an understanding of jet substructure}",
    eprint = "1307.0007",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2013-145, DCPT-13-86, IPPP-13-43, LPN13-036, MAN-HEP-2013-12",
    doi = "10.1007/JHEP09(2013)029",
    journal = "JHEP",
    volume = "09",
    pages = "029",
    year = "2013"
}


@article{Larkoski:2014wba,
    author = "Larkoski, Andrew J. and Marzani, Simone and Soyez, Gregory and Thaler, Jesse",
    title = "{Soft Drop}",
    eprint = "1402.2657",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4531, DCPT-14-24, IPPP-14-12",
    doi = "10.1007/JHEP05(2014)146",
    journal = "JHEP",
    volume = "05",
    pages = "146",
    year = "2014"
}


@article{Kardos:2020gty,
    author = "Kardos, Adam and Larkoski, Andrew J. and Tr\'ocs\'anyi, Zolt\'an",
    title = "{Groomed jet mass at high precision}",
    eprint = "2002.00942",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physletb.2020.135704",
    journal = "Phys. Lett. B",
    volume = "809",
    pages = "135704",
    year = "2020"
}


@article{Chang:2013rca,
    author = "Chang, Hsi-Ming and Procura, Massimiliano and Thaler, Jesse and Waalewijn, Wouter J.",
    title = "{Calculating Track-Based Observables for the LHC}",
    eprint = "1303.6637",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT-CTP-4449, MIT--CTP-4449",
    doi = "10.1103/PhysRevLett.111.102002",
    journal = "Phys. Rev. Lett.",
    volume = "111",
    pages = "102002",
    year = "2013"
}


@article{Chang:2013iba,
    author = "Chang, Hsi-Ming and Procura, Massimiliano and Thaler, Jesse and Waalewijn, Wouter J.",
    title = "{Calculating Track Thrust with Track Functions}",
    eprint = "1306.6630",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MIT--CTP-4476",
    doi = "10.1103/PhysRevD.88.034030",
    journal = "Phys. Rev. D",
    volume = "88",
    pages = "034030",
    year = "2013"
}


@article{Jaarsma:2022kdd,
    author = "Jaarsma, Max and Li, Yibei and Moult, Ian and Waalewijn, Wouter and Zhu, Hua Xing",
    title = "{Renormalization Group Flows for Track Function Moments}",
    eprint = "2201.05166",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "1",
    year = "2022"
}


@article{Li:2021zcf,
    author = "Li, Yibei and Moult, Ian and van Velzen, Solange Schrijnder and Waalewijn, Wouter J. and Zhu, Hua Xing",
    title = "{Extending Precision Perturbative QCD with Track Functions}",
    eprint = "2108.01674",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.128.182001",
    journal = "Phys. Rev. Lett.",
    volume = "128",
    number = "18",
    pages = "182001",
    year = "2022"
}


@article{Heinrich:2020ybq,
    author = "Heinrich, Gudrun",
    title = "{Collider Physics at the Precision Frontier}",
    eprint = "2009.00516",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KA-TP-13-2020, P3H-20-044",
    doi = "10.1016/j.physrep.2021.03.006",
    journal = "Phys. Rept.",
    volume = "922",
    pages = "1--69",
    year = "2021"
}


@article{Carli:2010rw,
    author = "Carli, Tancredi and Clements, Dan and Cooper-Sarkar, Amanda and Gwenlan, Claire and Salam, Gavin P. and Siegert, Frank and Starovoitov, Pavel and Sutton, Mark",
    title = "{A posteriori inclusion of parton density functions in NLO QCD final-state calculations at hadron colliders: The APPLGRID Project}",
    eprint = "0911.2985",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1140/epjc/s10052-010-1255-0",
    journal = "Eur. Phys. J. C",
    volume = "66",
    pages = "503--524",
    year = "2010"
}


@inproceedings{Kluge:2006xs,
    author = "Kluge, T. and Rabbertz, K. and Wobisch, M.",
    title = "{FastNLO: Fast pQCD calculations for PDF fits}",
    booktitle = "{14th International Workshop on Deep Inelastic Scattering}",
    eprint = "hep-ph/0609285",
    archivePrefix = "arXiv",
    reportNumber = "DESY-06-186, FERMILAB-CONF-06-352-E",
    doi = "10.1142/9789812706706_0110",
    pages = "483--486",
    month = "9",
    year = "2006"
}


@inproceedings{Campbell:2022qmc,
    author = "Campbell, J. M. and others",
    title = "{Event Generators for High-Energy Physics Experiments}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2203.11110",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CP3-22-12, DESY-22-042, FERMILAB-PUB-22-116-SCD-T, IPPP/21/51,
  JLAB-PHY-22-3576, KA-TP-04-2022, LA-UR-22-22126, LU-TP-22-12, MCNET-22-04,
  OUTP-22-03P, P3H-22-024, PITT-PACC 2207, UCI-TR-2022-02",
    month = "3",
    year = "2022"
}


@article{Jungman:1995df,
    author = "Jungman, Gerard and Kamionkowski, Marc and Griest, Kim",
    title = "{Supersymmetric dark matter}",
    eprint = "hep-ph/9506380",
    archivePrefix = "arXiv",
    reportNumber = "SU-4240-605, UCSD-PTH-95-02, IASSNS-HEP-95-14, CU-TP-677",
    doi = "10.1016/0370-1573(95)00058-5",
    journal = "Phys. Rept.",
    volume = "267",
    pages = "195--373",
    year = "1996"
}

@techreport{ATLASComputing,
      author        = "ATLAS Collaboration",
      title         = "{ATLAS Software and Computing HL-LHC Roadmap}",
      institution   = "CERN",
      address       = "Geneva",
      reportNumber  = "CERN-LHCC-2022-005, LHCC-G-182",
      month         = "Mar",
      year          = "2022",
      url           = "https://cds.cern.ch/record/2802918",
}

@article{CidVidal:2018eel,
    author = "Cid Vidal, Xabier and others",
    editor = "Dainese, Andrea and Mangano, Michelangelo and Meyer, Andreas B. and Nisati, Aleandro and Salam, Gavin and Vesterinen, Mika Anton",
    title = "{Report from Working Group 3}: {Beyond the Standard Model physics at the HL-LHC and HE-LHC}",
    eprint = "1812.07831",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-LPCC-2018-05",
    doi = "10.23731/CYRM-2019-007.585",
    journal = "CERN Yellow Rep. Monogr.",
    volume = "7",
    pages = "585--865",
    year = "2019"
}

@inproceedings{Boveia:2022jox,
    author = "Boveia, Antonio and others",
    title = "{Summarizing experimental sensitivities of collider experiments to dark matter models and comparison to other experiments}",
    booktitle = "{2022 Snowmass Summer Study}",
    eprint = "2206.03456",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2022"
}

@article{Albert:2022xla,
    author = "Albert, Andreas and others",
    title = "{Displaying dark matter constraints from colliders with varying simplified model parameters}",
    eprint = "2203.12035",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "3",
    year = "2022"
}

@article{10.1016/j.dark.2019.100365.Boveia.2020,
	abstract = {{This document summarises the proposal of the LHC Dark Matter Working Group on how to present LHC results on s -channel simplified dark matter models and to compare them to direct (indirect) detection experiments.}},
	author = {Boveia, Antonio and Buchmueller, Oliver and Busoni, Giorgio and D'Eramo, Francesco and Roeck, Albert De and Simone, Andrea De and Doglioni, Caterina and Dolan, Matthew J. and Genest, Marie-Helene and Hahn, Kristian and Haisch, Ulrich and Harris, Philip C. and Heisig, Jan and Ippolito, Valerio and Kahlhoefer, Felix and Khoze, Valentin V. and Kulkarni, Suchita and Landsberg, Greg and Lowette, Steven and Malik, Sarah and Mangano, Michelangelo and McCabe, Christopher and Mrenna, Stephen and Pani, Priscilla and Pree, Tristan du and Riotto, Antonio and Salek, David and Schmidt-Hoberg, Kai and Shepherd, William and Tait, Tim M.P. and Wang, Lian-Tao and Worm, Steven and Zurek, Kathryn},
	date-added = {2022-05-30 17:57:55 -0400},
	date-modified = {2022-05-30 17:57:55 -0400},
	doi = {10.1016/j.dark.2019.100365},
	issn = {2212-6864},
	journal = {Physics of the Dark Universe},
	pages = {100365},
	title = {{Recommendations on presenting LHC searches for missing transverse energy signals using simplified s -channel models of dark matter}},
	volume = {27},
	year = {2020},
	bdsk-url-1 = {https://doi.org/10.1016/j.dark.2019.100365}
	}

@article{10.1016/j.dark.2019.100377.Albert.2019,
	abstract = {{ Weakly-coupled TeV-scale particles may mediate the interactions between normal matter and dark matter. If so, the LHC would produce dark matter through these mediators, leading to the familiar ``mono- X '' search signatures, but the mediators would also produce signals without missing momentum via the same vertices involved in their production. This document from the LHC Dark Matter Working Group suggests how to compare searches for these two types of signals in case of vector and axial--vector mediators, based on a workshop that took place on September 19/20, 2016 and subsequent discussions. These suggestions include how to extend the spin-1 mediated simplified models already in widespread use to include lepton couplings. This document also provides analytic calculations of the relic density in the simplified models and reports an issue that arose when ATLAS and CMS first began to use preliminary numerical calculations of the dark matter relic density in these models.}},
	author = {Albert, Andreas and Backovi{\'c}, Mihailo and Boveia, Antonio and Buchmueller, Oliver and Busoni, Giorgio and Roeck, Albert De and Doglioni, Caterina and DuPree, Tristan and Fairbairn, Malcolm and Genest, Marie-H{\'e}l{\`e}ne and Gori, Stefania and Gustavino, Giuliano and Hahn, Kristian and Haisch, Ulrich and Harris, Philip C. and Hayden, Dan and Ippolito, Valerio and John, Isabelle and Kahlhoefer, Felix and Kulkarni, Suchita and Landsberg, Greg and Lowette, Steven and Mawatari, Kentarou and Riotto, Antonio and Shepherd, William and Tait, Tim M.P. and Tolley, Emma and Tunney, Patrick and Zaldivar, Bryan and Zinser, Markus},
	date-added = {2022-05-30 17:57:55 -0400},
	date-modified = {2022-05-30 17:57:55 -0400},
	doi = {10.1016/j.dark.2019.100377},
	issn = {2212-6864},
	journal = {Physics of the Dark Universe},
	pages = {100377},
	title = {{Recommendations of the LHC Dark Matter Working Group: Comparing LHC searches for dark matter mediators in visible and invisible decay channels and calculations of the thermal relic density}},
	volume = {26},
	year = {2019},
	bdsk-url-1 = {https://doi.org/10.1016/j.dark.2019.100377}
	}

@article{Han:2018wus,
    author = "Han, Tao and Mukhopadhyay, Satyanarayan and Wang, Xing",
    title = "{Electroweak Dark Matter at Future Hadron Colliders}",
    eprint = "1805.00015",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "PITT-PACC-1806",
    doi = "10.1103/PhysRevD.98.035026",
    journal = "Phys. Rev. D",
    volume = "98",
    number = "3",
    pages = "035026",
    year = "2018"
}

@Article{	  CMS:2010ifv,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Observation of Long-Range Near-Side Angular Correlations
		  in Proton-Proton Collisions at the LHC}",
  eprint	= "1009.4122",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-QCD-10-002, CERN-PH-EP-2010-031",
  doi		= "10.1007/JHEP09(2010)091",
  journal	= "JHEP",
  volume	= "09",
  pages		= "091",
  year		= "2010"
}

@Article{	  CMS:2012qk,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Observation of Long-Range Near-Side Angular Correlations
		  in Proton-Lead Collisions at the LHC}",
  eprint	= "1210.5482",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-12-005, CERN-PH-EP-2012-320, CMS-HIN-12-015",
  doi		= "10.1016/j.physletb.2012.11.025",
  journal	= "Phys. Lett. B",
  volume	= "718",
  pages		= "795--814",
  year		= "2013"
}

@Article{	  ATLAS:2012cix,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Observation of Associated Near-Side and Away-Side
		  Long-Range Correlations in $\sqrt{s_{NN}}$=5.02 TeV
		  Proton-Lead Collisions with the ATLAS Detector}",
  eprint	= "1212.5198",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2012-366",
  doi		= "10.1103/PhysRevLett.110.182302",
  journal	= "Phys. Rev. Lett.",
  volume	= "110",
  number	= "18",
  pages		= "182302",
  year		= "2013"
}

@Article{	  ALICE:2012eyl,
  author	= "Abelev, Betty and others",
  collaboration	= "ALICE",
  title		= "{Long-range angular correlations on the near and away side
		  in $p$-Pb collisions at $\sqrt{s_{NN}}=5.02$ TeV}",
  eprint	= "1212.2001",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2012-359",
  doi		= "10.1016/j.physletb.2013.01.012",
  journal	= "Phys. Lett. B",
  volume	= "719",
  pages		= "29--41",
  year		= "2013"
}

@Article{	  LHCb:2015coe,
  author	= "Aaij, Roel and others",
  collaboration	= "LHCb",
  title		= "{Measurements of long-range near-side angular correlations
		  in $\sqrt{s_{\text{NN}}}=5$TeV proton-lead collisions in
		  the forward region}",
  eprint	= "1512.00439",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "LHCB-PAPER-2015-040, CERN-PH-EP-2015-308",
  doi		= "10.1016/j.physletb.2016.09.064",
  journal	= "Phys. Lett. B",
  volume	= "762",
  pages		= "473--483",
  year		= "2016"
}

@Article{	  ATLAS:2017fur,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Evidence for light-by-light scattering in heavy-ion
		  collisions with the ATLAS detector at the LHC}",
  eprint	= "1702.01625",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-EP-2016-316",
  doi		= "10.1038/nphys4208",
  journal	= "Nature Phys.",
  volume	= "13",
  number	= "9",
  pages		= "852--858",
  year		= "2017"
}

@Article{	  CMS:2018erd,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Evidence for light-by-light scattering and searches for
		  axion-like particles in ultraperipheral PbPb collisions at
		  $\sqrt{s_\mathrm{NN}} =$ 5.02 TeV}",
  eprint	= "1810.04602",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-FSQ-16-012, CERN-EP-2018-271",
  doi		= "10.1016/j.physletb.2019.134826",
  journal	= "Phys. Lett. B",
  volume	= "797",
  pages		= "134826",
  year		= "2019"
}

@TechReport{	  Dainese:2703572,
  author	= "Dainese, Andrea and Mangano, Michelangelo and Meyer,
		  Andreas B and Nisati, Aleandro and Salam, Gavin and
		  Vesterinen, Mika Anton",
  title		= "{Report on the Physics at the HL-LHC, and Perspectives for
		  the HE-LHC}",
  institution	= "CERN",
  number	= "CERN-2019-007",
  year		= "2019",
  url		= "https://cds.cern.ch/record/2703572",
  doi		= "10.23731/CYRM-2019-007",
  type		= "CERN Yellow Report"
}

@Misc{		  ATLAS-ZDC-LHCC,
  author	= "{ATLAS Collaboration}",
  title		= "{A Radiation-Hard Zero Degree Calorimeter for ATLAS in the
		  HL-LHC era}",
  type		= "CERN-LHCC-2021-018, LHCC-P-019",
  year		= "2021",
  url		= "https://cds.cern.ch/record/2781150"
}

@TechReport{	  CMS-ZDC-TDR,
  author	= "Bashan, Y and Citron, Z and Cole, B and Grosse Perdekamp,
		  M and Hase, A and Koeth, T and Lantz, C and Lascio, S and
		  Longo, R and MacLean, D and Mignerey, A and Moyal, Y and
		  Murray, M and Nickel, M and Phipps, M and Popescu, S and
		  Santiago, N and Sickles, A and Shenkar, S and Steinberg, P
		  and Sudit, L and Tate, A and Wang, Q and Yang, S",
  title		= "{A Run 4 Zero Degree Calorimeter for CMS}",
  institution	= "CERN",
  address	= "Geneva",
  reportnumber	= "CERN-LHCC-2021-025, CMS-TDR-024",
  month		= "Nov",
  year		= "2021",
  url		= "https://cds.cern.ch/record/2791533",
  note		= "This is a joint project with the ATLAS heavy ion group"
}

@TechReport{	  CMS:2667167,
  author	= "{CMS Collaboration}",
  title		= "{A MIP Timing Detector for the CMS Phase-2 Upgrade}",
  institution	= "CERN",
  address	= "Geneva",
  reportnumber	= "CERN-LHCC-2019-003, CMS-TDR-020",
  month		= "Mar",
  year		= "2019",
  url		= "https://cds.cern.ch/record/2667167"
}

@TechReport{	  ALICE:2803563,
  author	= "ALICE, Collaboration",
  title		= "{Letter of intent for ALICE 3: A next generation heavy-ion
		  experiment at the LHC}",
  institution	= "CERN",
  address	= "Geneva",
  reportnumber	= "CERN-LHCC-2022-009, LHCC-I-038",
  month		= "Mar",
  year		= "2022",
  url		= "https://cds.cern.ch/record/2803563"
}

@Article{	  PHENIX:2015siv,
  author	= "Adare, A. and others",
  collaboration	= "PHENIX",
  title		= "{An Upgrade Proposal from the PHENIX Collaboration}",
  eprint	= "1501.06197",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  month		= "1",
  year		= "2015"
}

@Article{	  sPHENIX:2017lqb,
  author	= "Aidala, C. A. and others",
  collaboration	= "sPHENIX",
  title		= "{Design and Beam Test Results for the sPHENIX
		  Electromagnetic and Hadronic Calorimeter Prototypes}",
  eprint	= "1704.01461",
  archiveprefix	= "arXiv",
  primaryclass	= "physics.ins-det",
  reportnumber	= "FERMILAB-PUB-17-091-PPD",
  doi		= "10.1109/TNS.2018.2879047",
  journal	= "IEEE Trans. Nucl. Sci.",
  volume	= "65",
  number	= "12",
  pages		= "2901--2919",
  year		= "2018"
}

@Article{	  ATLAS:2010isq,
  collaboration	= "ATLAS",
  title		= "{Observation of a Centrality-Dependent Dijet Asymmetry in
		  Lead-Lead Collisions at $\sqrt{s_{NN}}=2.77$ TeV with the
		  ATLAS Detector at the LHC}",
  eprint	= "1011.6182",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  doi		= "10.1103/PhysRevLett.105.252303",
  journal	= "Phys. Rev. Lett.",
  volume	= "105",
  pages		= "252303",
  year		= "2010"
}

@Article{	  CMS:2011iwn,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Observation and studies of jet quenching in PbPb
		  collisions at nucleon-nucleon center-of-mass energy = 2.76
		  TeV}",
  eprint	= "1102.1957",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2011-001, CMS-HIN-10-004",
  doi		= "10.1103/PhysRevC.84.024906",
  journal	= "Phys. Rev. C",
  volume	= "84",
  pages		= "024906",
  year		= "2011"
}

@Article{	  CMS:2012ulu,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Jet momentum dependence of jet quenching in PbPb
		  collisions at $\sqrt{s_{NN}}=2.76$ TeV}",
  eprint	= "1202.5022",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-11-013, CERN-PH-EP-2012-042",
  doi		= "10.1016/j.physletb.2012.04.058",
  journal	= "Phys. Lett. B",
  volume	= "712",
  pages		= "176--197",
  year		= "2012"
}

@Article{	  CMS:2012ytf,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Studies of jet quenching using isolated-photon+jet
		  correlations in PbPb and $pp$ collisions at
		  $\sqrt{s_{NN}}=2.76$ TeV}",
  eprint	= "1205.0206",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-11-010, CERN-PH-EP-2012-089",
  doi		= "10.1016/j.physletb.2012.11.003",
  journal	= "Phys. Lett. B",
  volume	= "718",
  pages		= "773--794",
  year		= "2013"
}

@Article{	  CMS:2017ehl,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Study of jet quenching with isolated-photon+jet
		  correlations in PbPb and pp collisions at
		  $\sqrt{s_{_{\mathrm{NN}}}} =$ 5.02 TeV}",
  eprint	= "1711.09738",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-16-002, CERN-EP-2017-285",
  doi		= "10.1016/j.physletb.2018.07.061",
  journal	= "Phys. Lett. B",
  volume	= "785",
  pages		= "14--39",
  year		= "2018"
}

@Article{	  ATLAS:2018dgb,
  author	= "Aaboud, Morad and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of photon\textendash{}jet transverse momentum
		  correlations in 5.02 TeV Pb + Pb and $pp$ collisions with
		  ATLAS}",
  eprint	= "1809.07280",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-196",
  doi		= "10.1016/j.physletb.2018.12.023",
  journal	= "Phys. Lett. B",
  volume	= "789",
  pages		= "167--190",
  year		= "2019"
}

@Article{	  CMS:2017eqd,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Study of Jet Quenching with $Z+\text{jet}$ Correlations
		  in Pb-Pb and $pp$ Collisions at ${\sqrt{s}}_{NN}=5.02\text{
		  }\text{ }\mathrm{TeV}$}",
  eprint	= "1702.01060",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-15-013, CERN-EP-2017-002",
  doi		= "10.1103/PhysRevLett.119.082301",
  journal	= "Phys. Rev. Lett.",
  volume	= "119",
  number	= "8",
  pages		= "082301",
  year		= "2017"
}

@Article{	  ATLAS:2012tjt,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of the jet radius and transverse momentum
		  dependence of inclusive jet suppression in lead-lead
		  collisions at $\sqrt{s_{NN}}$= 2.76 TeV with the ATLAS
		  detector}",
  eprint	= "1208.1967",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2012-134",
  doi		= "10.1016/j.physletb.2013.01.024",
  journal	= "Phys. Lett. B",
  volume	= "719",
  pages		= "220--241",
  year		= "2013"
}

@Article{	  ATLAS:2014ipv,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Measurements of the Nuclear Modification Factor for Jets
		  in Pb+Pb Collisions at $\sqrt{s_{\mathrm{NN}}}=2.76$ TeV
		  with the ATLAS Detector}",
  eprint	= "1411.2357",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2014-172",
  doi		= "10.1103/PhysRevLett.114.072302",
  journal	= "Phys. Rev. Lett.",
  volume	= "114",
  number	= "7",
  pages		= "072302",
  year		= "2015"
}

@Article{	  CMS:2016uxf,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Measurement of inclusive jet cross sections in $pp$ and
		  PbPb collisions at $\sqrt{s_{NN}}=$ 2.76 TeV}",
  eprint	= "1609.05383",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-13-005, CERN-EP-2016-217",
  doi		= "10.1103/PhysRevC.96.015202",
  journal	= "Phys. Rev. C",
  volume	= "96",
  number	= "1",
  pages		= "015202",
  year		= "2017"
}

@Article{	  ATLAS:2018gwx,
  author	= "Aaboud, Morad and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of the nuclear modification factor for
		  inclusive jets in Pb+Pb collisions at
		  $\sqrt{s_\mathrm{NN}}=5.02$ TeV with the ATLAS detector}",
  eprint	= "1805.05635",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-105",
  doi		= "10.1016/j.physletb.2018.10.076",
  journal	= "Phys. Lett. B",
  volume	= "790",
  pages		= "108--128",
  year		= "2019"
}

@Article{	  CMS:2021vui,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{First measurement of large area jet transverse momentum
		  spectra in heavy-ion collisions}",
  eprint	= "2102.13080",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "FERMILAB-PUB-21-160-CMS, CMS-HIN-18-014, CERN-EP-2020-226",
  doi		= "10.1007/JHEP05(2021)284",
  journal	= "JHEP",
  volume	= "05",
  pages		= "284",
  year		= "2021"
}

@Article{	  ALICE:2015mjv,
  author	= "Adam, Jaroslav and others",
  collaboration	= "ALICE",
  title		= "{Measurement of jet suppression in central Pb-Pb
		  collisions at $\sqrt{s_{\rm NN}}$ = 2.76 TeV}",
  eprint	= "1502.01689",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2015-023",
  doi		= "10.1016/j.physletb.2015.04.039",
  journal	= "Phys. Lett. B",
  volume	= "746",
  pages		= "1--14",
  year		= "2015"
}

@Article{	  CMS:2015hkr,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Measurement of transverse momentum relative to dijet
		  systems in PbPb and pp collisions at $
		  \sqrt{s_{\mathrm{NN}}}=2.76 $ TeV}",
  eprint	= "1509.09029",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-14-010, CERN-PH-EP-2015-260",
  doi		= "10.1007/JHEP01(2016)006",
  journal	= "JHEP",
  volume	= "01",
  pages		= "006",
  year		= "2016"
}

@Article{	  CMS:2014jjt,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Measurement of Jet Fragmentation in PbPb and pp
		  Collisions at $\sqrt{s_{NN}}= 2.76$ TeV}",
  eprint	= "1406.0932",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-12-013, CERN-PH-EP-2014-100",
  doi		= "10.1103/PhysRevC.90.024908",
  journal	= "Phys. Rev. C",
  volume	= "90",
  number	= "2",
  pages		= "024908",
  year		= "2014"
}

@Article{	  ATLAS:2014dtd,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of inclusive jet charged-particle
		  fragmentation functions in Pb+Pb collisions at
		  $\sqrt{s_{NN}}=2.76$ TeV with the ATLAS detector}",
  eprint	= "1406.2979",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2014-101",
  doi		= "10.1016/j.physletb.2014.10.065",
  journal	= "Phys. Lett. B",
  volume	= "739",
  pages		= "320--342",
  year		= "2014"
}

@Article{	  ATLAS:2018bvp,
  author	= "Aaboud, Morad and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of jet fragmentation in Pb+Pb and $pp$
		  collisions at $\sqrt{s_{NN}} = 5.02$ TeV with the ATLAS
		  detector}",
  eprint	= "1805.05424",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-096",
  doi		= "10.1103/PhysRevC.98.024908",
  journal	= "Phys. Rev. C",
  volume	= "98",
  number	= "2",
  pages		= "024908",
  year		= "2018"
}

@Article{	  CMS:2013lhm,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Modification of Jet Shapes in PbPb Collisions at $\sqrt
		  {s_{NN}} = 2.76$ TeV}",
  eprint	= "1310.0878",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2013-189, CMS-HIN-12-002",
  doi		= "10.1016/j.physletb.2014.01.042",
  journal	= "Phys. Lett. B",
  volume	= "730",
  pages		= "243--263",
  year		= "2014"
}

@Article{	  CMS:2018mqn,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Observation of Medium-Induced Modifications of Jet
		  Fragmentation in Pb-Pb Collisions at $\sqrt{s_{NN}}=$ 5.02
		  TeV Using Isolated Photon-Tagged Jets}",
  eprint	= "1801.04895",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-16-014, CERN-EP-2017-337",
  doi		= "10.1103/PhysRevLett.121.242301",
  journal	= "Phys. Rev. Lett.",
  volume	= "121",
  number	= "24",
  pages		= "242301",
  year		= "2018"
}

@Article{	  CMS:2018jco,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Jet Shapes of Isolated Photon-Tagged Jets in Pb-Pb and pp
		  Collisions at $\sqrt{s_\mathrm{NN}} =$ 5.02 TeV}",
  eprint	= "1809.08602",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-18-006, CERN-EP-2018-249",
  doi		= "10.1103/PhysRevLett.122.152001",
  journal	= "Phys. Rev. Lett.",
  volume	= "122",
  number	= "15",
  pages		= "152001",
  year		= "2019"
}

@Article{	  ATLAS:2020wmg,
  author	= "Aad, Georges and others",
  collaboration	= "ATLAS",
  title		= "{Medium-Induced Modification of $Z$-Tagged Charged
		  Particle Yields in $Pb+Pb$ Collisions at 5.02 TeV with the
		  ATLAS Detector}",
  eprint	= "2008.09811",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2020-148",
  doi		= "10.1103/PhysRevLett.126.072301",
  journal	= "Phys. Rev. Lett.",
  volume	= "126",
  number	= "7",
  pages		= "072301",
  year		= "2021"
}

@Article{	  CMS:2021otx,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Using Z Boson Events to Study Parton-Medium Interactions
		  in Pb-Pb Collisions}",
  eprint	= "2103.04377",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-19-006, CERN-EP-2021-014",
  doi		= "10.1103/PhysRevLett.128.122301",
  journal	= "Phys. Rev. Lett.",
  volume	= "128",
  number	= "12",
  pages		= "122301",
  year		= "2022"
}

@Article{	  CMS:2020plq,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of quark- and gluon-like jet fractions using
		  jet charge in PbPb and pp collisions at 5.02 TeV}",
  eprint	= "2004.00602",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-18-018, CERN-EP-2020-019",
  doi		= "10.1007/JHEP07(2020)115",
  journal	= "JHEP",
  volume	= "07",
  pages		= "115",
  year		= "2020"
}

@Article{	  CMS:2017qlm,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of the Splitting Function in $pp$ and Pb-Pb
		  Collisions at $\sqrt{s_{_{\mathrm{NN}}}} =$ 5.02 TeV}",
  eprint	= "1708.09429",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-16-006, CERN-EP-2017-205",
  doi		= "10.1103/PhysRevLett.120.142302",
  journal	= "Phys. Rev. Lett.",
  volume	= "120",
  number	= "14",
  pages		= "142302",
  year		= "2018"
}

@Article{	  CMS:2018fof,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of the groomed jet mass in PbPb and pp
		  collisions at $ \sqrt{s_{\mathrm{NN}}}=5.02 $ TeV}",
  eprint	= "1805.05145",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-16-024, CERN-EP-2018-097",
  doi		= "10.1007/JHEP10(2018)161",
  journal	= "JHEP",
  volume	= "10",
  pages		= "161",
  year		= "2018"
}

@Article{	  ALICE:2019ykw,
  author	= "Acharya, Shreyasi and others",
  collaboration	= "ALICE",
  title		= "{Exploration of jet substructure using iterative
		  declustering in pp and Pb\textendash{}Pb collisions at LHC
		  energies}",
  eprint	= "1905.02512",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2019-087",
  doi		= "10.1016/j.physletb.2020.135227",
  journal	= "Phys. Lett. B",
  volume	= "802",
  pages		= "135227",
  year		= "2020"
}

@Article{	  ALICE:2018dxf,
  author	= "Acharya, Shreyasi and others",
  collaboration	= "ALICE",
  title		= "{Medium modification of the shape of small-radius jets in
		  central Pb-Pb collisions at $\sqrt{s_{\mathrm {NN}}} =
		  2.76\,\rm{TeV}$}",
  eprint	= "1807.06854",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-201",
  doi		= "10.1007/JHEP10(2018)139",
  journal	= "JHEP",
  volume	= "10",
  pages		= "139",
  year		= "2018"
}

@Article{	  CMS:2017uoy,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of the ${B}^{\pm}$ Meson Nuclear Modification
		  Factor in Pb-Pb Collisions at $\sqrt{{s}_{NN}}=5.02\text{
		  }\text{ }\mathrm{TeV}$}",
  eprint	= "1705.04727",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-16-011, CERN-EP-2017-076",
  doi		= "10.1103/PhysRevLett.119.152301",
  journal	= "Phys. Rev. Lett.",
  volume	= "119",
  number	= "15",
  pages		= "152301",
  year		= "2017"
}

@Article{	  CMS:2018eso,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of B$^0_\mathrm{s}$ meson production in pp
		  and PbPb collisions at $\sqrt{s_\mathrm{NN}} =$ 5.02 TeV}",
  eprint	= "1810.03022",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-17-008, CERN-EP-2018-257",
  doi		= "10.1016/j.physletb.2019.07.014",
  journal	= "Phys. Lett. B",
  volume	= "796",
  pages		= "168--190",
  year		= "2019"
}

@Article{	  ALICE:2018lyv,
  author	= "Acharya, S. and others",
  collaboration	= "ALICE",
  title		= "{Measurement of D$^{0}$, D$^{+}$, D$^{*+}$ and D$_{s}^{+}$
		  production in Pb-Pb collisions at $
		  \sqrt{{\mathrm{s}}_{\mathrm{NN}}}=5.02 $ TeV}",
  eprint	= "1804.09083",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-066",
  doi		= "10.1007/JHEP10(2018)174",
  journal	= "JHEP",
  volume	= "10",
  pages		= "174",
  year		= "2018"
}

@Article{	  CMS:2017qjw,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Nuclear modification factor of D$^0$ mesons in PbPb
		  collisions at $\sqrt{s_\mathrm{NN}} = 5.02$ TeV}",
  eprint	= "1708.04962",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-16-001, CERN-EP-2017-186",
  doi		= "10.1016/j.physletb.2018.05.074",
  journal	= "Phys. Lett. B",
  volume	= "782",
  pages		= "474--496",
  year		= "2018"
}

@Article{	  ALICE:2015vxz,
  author	= "Adam, Jaroslav and others",
  collaboration	= "ALICE",
  title		= "{Transverse momentum dependence of D-meson production in
		  Pb-Pb collisions at $ \sqrt{{\mathrm{s}}_{\mathrm{NN}}}=$
		  2.76 TeV}",
  eprint	= "1509.06888",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2015-252",
  doi		= "10.1007/JHEP03(2016)081",
  journal	= "JHEP",
  volume	= "03",
  pages		= "081",
  year		= "2016"
}

@Article{	  ALICE:2021mgk,
  author	= "Acharya, Shreyasi and others",
  collaboration	= "ALICE",
  title		= "{Measurement of beauty and charm production in pp
		  collisions at $ \sqrt{s} $ = 5.02 TeV via non-prompt and
		  prompt D mesons}",
  eprint	= "2102.13601",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2021-034",
  doi		= "10.1007/JHEP05(2021)220",
  journal	= "JHEP",
  volume	= "05",
  pages		= "220",
  year		= "2021"
}

@Article{	  CMS:2018bwt,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Studies of Beauty Suppression via Nonprompt $D^0$ Mesons
		  in Pb-Pb Collisions at $Q^2 = 4$ $\rm GeV^2$}",
  eprint	= "1810.11102",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-16-016, CERN-EP-2018-264",
  doi		= "10.1103/PhysRevLett.123.022001",
  journal	= "Phys. Rev. Lett.",
  volume	= "123",
  number	= "2",
  pages		= "022001",
  year		= "2019"
}

@Article{	  CMS:2017exb,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Measurement of prompt and nonprompt $\mathrm{J}/{\psi }$
		  production in $\mathrm {p}\mathrm {p}$ and $\mathrm
		  {p}\mathrm {Pb}$ collisions at $\sqrt{s_{\mathrm {NN}}}
		  =5.02\,\text {TeV} $}",
  eprint	= "1702.01462",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-14-009, CERN-EP-2017-009",
  doi		= "10.1140/epjc/s10052-017-4828-3",
  journal	= "Eur. Phys. J. C",
  volume	= "77",
  number	= "4",
  pages		= "269",
  year		= "2017"
}

@Article{	  ATLAS:2018hqe,
  author	= "Aaboud, Morad and others",
  collaboration	= "ATLAS",
  title		= "{Prompt and non-prompt $J/\psi $ and $\psi (2\mathrm {S})$
		  suppression at high transverse momentum in $5.02~\mathrm
		  {TeV}$ Pb+Pb collisions with the ATLAS experiment}",
  eprint	= "1805.04077",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-EP-2018-049",
  doi		= "10.1140/epjc/s10052-018-6219-9",
  journal	= "Eur. Phys. J. C",
  volume	= "78",
  number	= "9",
  pages		= "762",
  year		= "2018"
}

@Article{	  CMS:2011all,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Indications of suppression of excited $\Upsilon$ states
		  in PbPb collisions at $\sqrt{S_{NN}}$ = 2.76 TeV}",
  eprint	= "1105.4894",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2011-074, CMS-HIN-11-007",
  doi		= "10.1103/PhysRevLett.107.052302",
  journal	= "Phys. Rev. Lett.",
  volume	= "107",
  pages		= "052302",
  year		= "2011"
}

@Article{	  CMS:2012bms,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Suppression of non-prompt $J/\psi$, prompt $J/\psi$, and
		  Y(1S) in PbPb collisions at $\sqrt{s_{NN}}=2.76$ TeV}",
  eprint	= "1201.5069",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-10-006, CERN-PH-EP-2011-170",
  doi		= "10.1007/JHEP05(2012)063",
  journal	= "JHEP",
  volume	= "05",
  pages		= "063",
  year		= "2012"
}

@Article{	  CMS:2012gvv,
  author	= "Chatrchyan, Serguei and others",
  collaboration	= "CMS",
  title		= "{Observation of Sequential Upsilon Suppression in PbPb
		  Collisions}",
  eprint	= "1208.2826",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-11-011, CERN-PH-EP-2012-228",
  doi		= "10.1103/PhysRevLett.109.222301",
  journal	= "Phys. Rev. Lett.",
  volume	= "109",
  pages		= "222301",
  year		= "2012",
  note		= "[Erratum: Phys.Rev.Lett. 120, 199903 (2018)]"
}

@Article{	  CMS:2016rpc,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Suppression of $\Upsilon(1S), \Upsilon(2S)$ and
		  $\Upsilon(3S)$ production in PbPb collisions at
		  $\sqrt{s_{\rm NN}}$ = 2.76 TeV}",
  eprint	= "1611.01510",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-15-001, CERN-EP-2016-248",
  doi		= "10.1016/j.physletb.2017.04.031",
  journal	= "Phys. Lett. B",
  volume	= "770",
  pages		= "357--379",
  year		= "2017"
}

@Article{	  ATLAS:2010xzb,
  author	= "Aad, G. and others",
  collaboration	= "ATLAS",
  title		= "{Measurement of the centrality dependence of
		  J/\ensuremath{\psi} yields and observation of Z production
		  in lead\textendash{}lead collisions with the ATLAS detector
		  at the LHC}",
  eprint	= "1012.5419",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2010-090",
  doi		= "10.1016/j.physletb.2011.02.006",
  journal	= "Phys. Lett. B",
  volume	= "697",
  pages		= "294--312",
  year		= "2011"
}

@Article{	  ALICE:2012jsl,
  author	= "Abelev, Betty and others",
  collaboration	= "ALICE",
  title		= "{$J/\psi$ suppression at forward rapidity in Pb-Pb
		  collisions at $\sqrt{s_{NN}}=2.76$ TeV}",
  eprint	= "1202.1383",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CERN-PH-EP-2012-012",
  doi		= "10.1103/PhysRevLett.109.072301",
  journal	= "Phys. Rev. Lett.",
  volume	= "109",
  pages		= "072301",
  year		= "2012"
}

@Article{	  CMS:2014vjg,
  author	= "Khachatryan, Vardan and others",
  collaboration	= "CMS",
  title		= "{Measurement of Prompt $\psi(2S) \to J/\psi$ Yield Ratios
		  in Pb-Pb and $p-p$ Collisions at $\sqrt {s_{NN}}=$ 2.76
		  TeV}",
  eprint	= "1410.1804",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CMS-HIN-12-007, CERN-PH-EP-2014-240",
  doi		= "10.1103/PhysRevLett.113.262301",
  journal	= "Phys. Rev. Lett.",
  volume	= "113",
  number	= "26",
  pages		= "262301",
  year		= "2014"
}

@Article{	  ALICE:2015jrl,
  author	= "Adam, Jaroslav and others",
  collaboration	= "ALICE",
  title		= "{Differential studies of inclusive J/\ensuremath{\psi} and
		  \ensuremath{\psi}(2S) production at forward rapidity in
		  Pb-Pb collisions at $ \sqrt{s_{\mathrm{NN}}}=2.76 $ TeV}",
  eprint	= "1506.08804",
  archiveprefix	= "arXiv",
  primaryclass	= "nucl-ex",
  reportnumber	= "CERN-PH-EP-2015-157",
  doi		= "10.1007/JHEP05(2016)179",
  journal	= "JHEP",
  volume	= "05",
  pages		= "179",
  year		= "2016"
}

@TechReport{	  FTR-18-025,
  title		= "{Performance of jet quenching measurements in pp and PbPb
		  collisions with CMS at the HL-LHC}",
  author	= "{CMS Collaboration}",
  institution	= "CERN",
  number	= "CMS-PAS-FTR-18-025",
  year		= "2018",
  reportnumber	= "CMS-PAS-FTR-18-025",
  url		= "http://cds.cern.ch/record/2651892",
  type		= " CMS Physics Analysis Summary"
}


@Booklet{	  ATL-PHYS-PUB-2018-019,
  author	= "{ATLAS Collaboration}",
  title		= "{Projections for ATLAS Measurements of Jet Modifications
		  in Pb+Pb Collisions in LHC Runs 3 and 4}",
  howpublished	= "{ATL-PHYS-PUB-2018-019}",
  url		= "https://cds.cern.ch/record/2644406",
  year		= "2018"
}


@Article{	  Aronson:2017ymv,
  author	= "Aronson, Samuel and Borras, Evan and Odegard, Brunel and
		  Sharma, Rishi and Vitev, Ivan",
  title		= "{Collisional and thermal dissociation of $J/\psi$ and
		  $\Upsilon$ states at the LHC}",
  eprint	= "1709.02372",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ph",
  doi		= "10.1016/j.physletb.2018.01.038",
  journal	= "Phys. Lett. B",
  volume	= "778",
  pages		= "384--391",
  year		= "2018"
}

@Article{	  Kopeliovich:2014una,
  author	= "Kopeliovich, B. Z. and Potashnikova, I. K. and Schmidt,
		  Ivan and Siddikov, M.",
  title		= "{Survival of charmonia in a hot environment}",
  eprint	= "1409.5147",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ph",
  reportnumber	= "USM-TH-329",
  doi		= "10.1103/PhysRevC.91.024911",
  journal	= "Phys. Rev. C",
  volume	= "91",
  number	= "2",
  pages		= "024911",
  year		= "2015"
}

@Article{	  Du:2017qkv,
  author	= "Du, Xiaojian and Rapp, Ralf and He, Min",
  title		= "{Color Screening and Regeneration of Bottomonia in
		  High-Energy Heavy-Ion Collisions}",
  eprint	= "1706.08670",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ph",
  doi		= "10.1103/PhysRevC.96.054901",
  journal	= "Phys. Rev. C",
  volume	= "96",
  number	= "5",
  pages		= "054901",
  year		= "2017"
}

@TechReport{	  FTR-18-024,
  title		= "{Open heavy flavor and quarkonia in heavy ion collisions
		  at HL-LHC}",
  author	= "{CMS Collaboration}",
  institution	= "CERN",
  number	= "CMS-PAS-FTR-18-024",
  year		= "2018",
  reportnumber	= "CMS-PAS-FTR-18-024",
  url		= "http://cds.cern.ch/record/2650897",
  type		= " CMS Physics Analysis Summary"
}

@TechReport{	  FTR-18-026,
  title		= "{Predictions on the precision achievable for small system
		  flow observables in the context of HL-LHC}",
  author	= "{CMS Collaboration}",
  institution	= "CERN",
  number	= "CMS-PAS-FTR-18-026",
  year		= "2018",
  reportnumber	= "CMS-PAS-FTR-18-026",
  url		= "http://cds.cern.ch/record/2650773",
  type		= " CMS Physics Analysis Summary"
}

@TechReport{	  FTR-18-027,
  title		= "{Constraining nuclear parton distributions with heavy ion
		  collisions at the HL-LHC with the CMS experiment}",
  author	= "{CMS Collaboration}",
  institution	= "CERN",
  number	= "CMS-PAS-FTR-18-027",
  year		= "2018",
  reportnumber	= "CMS-PAS-FTR-18-027",
  url		= "http://cds.cern.ch/record/2652030",
  type		= " CMS Physics Analysis Summary"
}


@TechReport{	  ATL-PHYS-PUB-2018-020,
  author	= {{ATLAS collaboration}},
  title		= {{Projections for ATLAS Measurements of Bulk Properties of
		  Pb+Pb, $p$+Pb, and $pp$ Collisions in LHC Runs 3 and 4}},
  year		= 2018,
  month		= {Oct},
  address	= {Geneva},
  url		= {http://cds.cern.ch/record/2644407},
  institution	= {CERN},
  collaboration	= {ATLAS},
  reportnumber	= {ATL-PHYS-PUB-2018-020}
}

@Article{	  CMS:2021znk,
  author	= "Sirunyan, Albert M and others",
  collaboration	= "CMS",
  title		= "{Evidence for X(3872) in Pb-Pb Collisions and Studies of
		  its Prompt Production at $\sqrt {s_{NN}}$=5.02\,\,TeV}",
  eprint	= "2102.13048",
  archiveprefix	= "arXiv",
  primaryclass	= "hep-ex",
  reportnumber	= "CMS-HIN-19-005, CERN-EP-2021-023",
  doi		= "10.1103/PhysRevLett.128.032001",
  journal	= "Phys. Rev. Lett.",
  volume	= "128",
  number	= "3",
  pages		= "032001",
  year		= "2022"
}

@article{LHCb:2020sey,
    author = "Aaij, Roel and others",
    collaboration = "LHCb",
    title = "{Observation of Multiplicity Dependent Prompt $\chi_{c1}(3872)$ and $\psi(2S)$ Production in $pp$ Collisions}",
    eprint = "2009.06619",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "LHCb-PAPER-2020-023, CERN-EP-2020-161",
    doi = "10.1103/PhysRevLett.126.092001",
    journal = "Phys. Rev. Lett.",
    volume = "126",
    number = "9",
    pages = "092001",
    year = "2021"
}

@article{Feng:2022inv,
    author = "Feng, Jonathan L. and others",
    title = "{The Forward Physics Facility at the High-Luminosity LHC}",
    eprint = "2203.05090",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "UCI-TR-2022-01, CERN-PBC-Notes-2022-001,
  FERMILAB-PUB-22-094-ND-SCD-T, INT-PUB-22-006, BONN-TH-2022-04",
    month = "3",
    year = "2022"
}



==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

